Sharing Equality is Linear

The $\lambda$-calculus is a handy formalism to specify the evaluation of higher-order programs. It is not very handy, however, when one interprets the specification as an execution mechanism, because terms can grow exponentially with the number of $\beta$-steps. This is why implementations of functional languages and proof assistants always rely on some form of sharing of subterms. These frameworks however do not only evaluate $\lambda$-terms, they also have to compare them for equality. In presence of sharing, one is actually interested in the equality---or more precisely $\alpha$-conversion---of the underlying unshared $\lambda$-terms. The literature contains algorithms for such a sharing equality, that are polynomial in the sizes of the shared terms. This paper improves the bounds in the literature by presenting the first linear time algorithm. As others before us, we are inspired by Paterson and Wegman's algorithm for first-order unification, itself based on representing terms with sharing as DAGs, and sharing equality as bisimulation of DAGs.

==> 99-01-alpha.tex <==
% !TEX root = main.tex
\section{$\alpha$-equivalence} \label{sect:alpha}

\begin{definition}[Free Variables] \label{def:fv}
Let $\tm,\tmtwo$ be named terms,
and $\var$ be a variable.
We define the free variables of a term by induction on the structure of terms:
\begin{enumerate}
 \item\label{fv:var} $\fv\var \defeq \set\var$;
 \item\label{fv:app} $\fv{\tm \tmtwo} \defeq \fv\tm \cup \fv \tmtwo$;
 \item\label{fv:lam} $\fv{\la\var\tm} \defeq \fv\tm \setminus \set\var$.
\end{enumerate}
\end{definition}

\begin{definition}[Variables] \label{def:av}
Let $\tm,\tmtwo$ be named terms,
and $\var$ be a variable.
We define the variables of a term by induction on the structure of terms:
\begin{enumerate}
 \item\label{av:var} $\av\var \defeq \set\var$;
 \item\label{av:app} $\av{\tm \tmtwo} \defeq \av\tm \cup \av \tmtwo$;
 \item\label{av:lam} $\av{\la\var\tm} \defeq \av\tm \cup \set\var$.
\end{enumerate}
\end{definition}

\begin{definition}[(Capture-Avoiding) Substitution]
  Let $\tm,\tmtwo,\tmthree$ be named terms,
  and $\var,\vartwo,\varthree$ be variables.
  We define the capture-avoiding substitution by induction on the structure of terms:
\begin{enumerate}
 \item\label{sub:vareq} $\var\isub\var\tmtwo \defeq \tmtwo$;
 \item\label{sub:vardif} $\vartwo \isub\var\tmtwo \defeq \vartwo$;
 \item\label{sub:app} $(\tm \tmtwo)\isub\var\tmthree \defeq \tm\isub\var\tmthree \tmtwo \isub\var\tmthree$;
 \item\label{sub:lameq} $(\la\var\tm) \isub\var\tmtwo \defeq \la\var\tm$;
 \item\label{???} $(\la\vartwo\tm) \isub\var\tmtwo \defeq \la\vartwo\tm\isub\var\tmtwo$ when $\vartwo \notin \set\var \cup \fv\tmtwo$;
 \item\label{sub:lamdiff} $(\la\vartwo\tm) \isub\var\tmtwo \defeq \la\varthree\tm\isub\vartwo\varthree \isub\var\tmtwo$ with $\varthree \notin \av\tm \cup \set\var \cup \fv\tmtwo$;
\end{enumerate}
\end{definition}


==> figure_algorithm.tex <==
% !TEX root = main.tex
\begin{algorithm}
 \SetArgSty{textrm}
 \SetAlgoLined
 % \DontPrintSemicolon

 \KwData{an initial state}
 \KwResult{either \FAIL or a final state}
 \BlankLine

 \SetKwProg{myfinish}{Procedure}{}{}
 \SetKwProg{mypush}{Procedure}{}{}
 \SetKwProg{mypropagate}{Procedure}{}{}
 \SetKwProg{mymain}{Procedure}{}{}

 \SetKw{and}{and}
 \SetKw{nott}{not}

 \mymain{\main{}}{
 % \tcp{build sharing equivalence}
 \nl \lWhile{there is any alive node $\node$}{\fin{$\node$}\label{alg_start}}
 % \tcp{check if it is a $\l$-sharing equivalence}
 % \nl \label{alg:check_var_nodes}\While{$\node$ is a var-node}{
 % $\nodetwo \defeq \pointer\node$\;
 % \If{$\node\neq\nodetwo$}{
 % \nl \lIf{$\binder \node$ is $\cundefined$ {\normalfont\textbf{or}} $\binder{\nodetwo}$ is $\cundefined$ \label{alg:propagate.failUno}}{\FAIL}
 % \nl \lElseIf{$\pointer{\binder\node} \neq \pointer{\binder {\nodetwo}}$}{\label{alg:propagate.failDue}\FAIL}
 % }
 % }
 }
 \BlankLine
 \myfinish{\fin{$\wcan$}}{
 $\stack \defeq \emptyset$\label{alg_create}\;
 \leIf{$\pointer \wcan$ is $\cundefined$\label{alg_if_undefi}}{%
 $\pointer \wcan \leftarrow \wcan$\label{alg_assign_canoni}%
 }{%
 \FAIL \label{alg_push_faili}%
 } \nl%
 \lWhile{$\wcan$ has some alive parent $\node$}
 {\label{alg6i}$\fin{\node}$}

 \nl \While{there is an undirected query edge $(\wcan,\node)$\label{alg_while3i}}{%
 \push{$\stack$, $\wcan$, $\node$}\label{alg7i}\;
 delete undirected query edge $(\wcan,\node)$\;
 }

 \While{\nott $\stack$.empty()\label{alg_while1}}{
 $\sthead\defeq \stack$.head()\; \label{alg_pop}
 \nl \lWhile{$\sthead$ has some alive parent $\node$}{$\fin{\node}$\label{alg6}}
 \nl \While{there is an undirected query edge $(\sthead,\node)$\label{alg_while3}}{
 \push{$\stack$, $\wcan$, $\node$}\label{alg7}\;
 delete undirected query edge $(\sthead,\node)$\label{alg8}\;
 }
 \nl $\stack$.pop()\label{alg11}\label{alg_end_while1}\;
 mark $\sthead$ dead\;
 }
 \nl mark $\wcan$ dead\label{alg12}\;
 }

 \BlankLine
 \mypush{\push{$\stack$, $\wcan$, $\node$}}{
 \uIf{$\pointer \node$ is $\cundefined$\label{alg_if_undef}}{
 \nl       $\pointer \node \defeq \wcan$\label{alg_assign_canon}\;
 \nl       $\stack$.push($\node$)\label{alg_push}\;
 \nl \lIf{$\wcan$, $\node$ have different labels}{\FAIL\label{alg_clash}}
 \If{$\wcan$ and $\node$ have children resp. $\wcan_1,\wcan_2$ and $\node_1,\node_2$}{
 \nl       create undirected query edges $(\wcan_1, \node_1)$ and $(\wcan_2, \node_2)$\label{alg_prop_app}\;}
 }
 \nl \lElseIf{$\pointer \node \neq \wcan$}{\FAIL\label{alg_push_fail}}
 }

 \caption{\Core sharing check}
 \label{alg:sharing-check}
\end{algorithm}


==> notations/ac.tex <==
\makeatletter\ifcsname acpkgalready\endcsname\else%
\@namedef{acpkgalready}{yep}

\usepackage{listofitems}

\newcommand\newnotation[2]{%
  \ifcsname mynotation@#1\endcsname
   #2
  \else%
  \fi%
}
% \NewEnviron{Notation}[1]{%
%   \ifcsname mynotation@#1\endcsname
%    #1
%   \else%
%   \fi%
% }

\newcommand\@usenotation[1]{%
 \@namedef{mynotation@#1}{okay}%
}

\newcommand\usenotation[2][]{
 \setsepchar{,}
 \readlist*\nots{#1}
 \foreachitem\x\in\nots[]{\expandafter\@usenotation{\x}}
 \readlist*\paths{#2}
 \foreachitem\x\in\paths[]{\input\x}
}

% Finally, call \usenotation to capture
% the upcoming notation names
\fi\makeatother\usenotation


==> notations/general.tex <==
\newnotation{general}{
  \newcommand\defeq\coloneqq
  \newcommand\eqdef{=:}
  \newcommand\grameq{::=}
  \newcommand\ie{\textit{i.e.}\xspace}
  \newcommand\eg{\textit{e.g.}\xspace}
  \newcommand\ih{\textit{i.h.}\xspace}
  \newcommand\den[1]{\left\llbracket#1\right\rrbracket}
  \DeclarePairedDelimiter{\set}{\{}{\}}
}

\newnotation{ac}{
  \newcommand\ac[1]{\color{violet}#1\color{black}}
  \newcommand\TODO[1]{\textbf{\textcolor{red}{\texttt{[TODO]} #1}}}
}


==> notations/notations.tex <==

\newnotation{type-option}{
  % Option type (None, Some)
  \newcommand{\None}{\texttt{None}}
  \newcommand{\Some}{\texttt{Some}\,}
}

\makeatletter
\newnotation{ac-termgraph-paths}{
% Arrows
\newcommand{\fixed@sra}{$\vrule height 2\fontdimen22\textfont2 width 0pt\shortrightarrow$}
\newcommand{\shortarrow}[1]{%
  \mathrel{\text{\rotatebox[origin=c]{\numexpr#1*45}{\fixed@sra}}}
}
\renewcommand{\swarrow}{\shortarrow{5}}
\renewcommand{\downarrow}{\shortarrow{6}}
\renewcommand{\searrow}{\shortarrow{7}}
\newcommand{\pempty}{\epsilon}
\newcommand{\pcons}[2]{#2\cdot#1}
\newcommand{\pappend}[1]{#1\cdot}
\newcommand{\proot}[1]{\mathcal{S}tart(#1)}
\newcommand{\pdown}{{\downarrow}}
\newcommand{\pleft}{{\swarrow}}
\newcommand{\pright}{{\searrow}}
\newcommand{\pback}{{\circlearrowright}}
\newcommand{\tra}{\tau}
\newcommand{\trax}{\tra'}
\newcommand{\traxx}{\tra''}
% \newcommand{\dir}{d}
\newcommand{\Path}[2]{#2\xrsquigarrow{#1}}
% \newcommand{\Pathp}[2]{\Path{(#1)}{#2}}
\newcommand\Pathp\Path
}
\makeatother

\newnotation{ac-termgraph-inferences}{
% Rules
\newcommand{\RuleAux}[1]{(#1)}
\renewcommand{\RuleAux}[1]{\colorbox{black!10}{%
\parbox[c][0.5em][c]{0.7em}{%
\makebox[0.7em]{\textcolor{black}{#1}}%
}%
% \parbox[c][0.6em][c]{0.4em}{\centering#1}
 % \makebox[0.9em]{\textcolor{black}{#1}}%
 }}
\newcommand{\RuleAppl}{\RuleAux{$\pleft$}}
\newcommand{\RuleAppr}{\RuleAux{$\pright$}}
\newcommand{\RuleAbs}{\RuleAux{$\pdown$}}
% \newcommand{\RuleFV}{fv}
\newcommand{\RuleBV}{\RuleAux{$\pback$}}
\newcommand{\RuleRefl}{\RuleAux{{\tiny$\bullet$}}}
\newcommand{\RuleSym}{\RuleAux{$\shortarrow{0}\!\!\!\!\!\shortarrow{4}$}}
\newcommand{\RuleTrans}{\RuleAux{$\shortarrow{0}\!\!\!\shortarrow{0}$}}
}


\newnotation{ac-termgraph-relations}{
% Relations and Closures
  \newcommand{\Rel}{\mathrel{\mathcal{R}}} % Relation
  \newcommand{\Relx}{\Rel'}
  \newcommand{\Relxx}{\Rel''}
  \newcommand{\Bis}{\mathrel{\mathcal{B}}} % Bisimulation
  \newcommand{\Que}{\mathrel{\mathcal{Q}}} % Query
  \newcommand{\DownClos}[1]{#1^{\Downarrow}}
  \newcommand{\DownEquivClos}[1]{#1^{\#}}
}

\newnotation{termgraph}{
  \newcommand{\LabelBVar}{\texttt{BVar}}
  \newcommand{\LabelFVar}{\texttt{FVar}}
  \newcommand{\LabelVar}{\texttt{Var}}
  \newcommand{\LabelApp}{\texttt{App}}
  \newcommand{\LabelAbs}{\texttt{Abs}}
  \newcommand{\NodeApp}[2]{\LabelApp\texttt{(}#1\texttt{,}#2\texttt{)}}
  \newcommand{\NodeAbs}[1]{\LabelAbs\texttt{(}#1\texttt{)}}
  \newcommand{\NodeBVar}[1]{\texttt{BVar}(#1)}
  \newcommand{\NodeFVar}[1]{\texttt{Atom}(#1)}
  \newcommand{\nbvar}[1]{\LabelVar\texttt{(}#1\texttt{)}}
  \newcommand\nfvar{\nbvar{}}%{\texttt{Atom(}#1\texttt{)}}
  \newcommand{\napp}{\NodeApp}
  \newcommand{\nabs}{\NodeAbs}
  \newcommand{\noder}{r}%\texttt{n}}
  \newcommand{\noderx}{r'}%\texttt{n}}
  \newcommand{\node}{n}%\texttt{n}}
  \newcommand{\nodetwo}{m}
  \newcommand{\nodethree}{p}
  \newcommand{\nodefour}{q}
  \newcommand{\nodex}{m}%\texttt{m}}
  \newcommand{\nodexx}{p}%\texttt{p}}
  \newcommand{\nodel}{l}%\texttt{l}}
  \newcommand{\nodelx}{l'}%\texttt{l}'}
  \newcommand{\nodelxx}{l''}%\texttt{l}''}
  
  \newcommand\lan{node}%{$\lambda$-node}
  \newcommand\ladag{$\lambda$-graph}
  \newcommand\lac{$\lambda$-calculus}
  \newcommand\latree{$\lambda$-tree}
}

\newnotation{lambda-calculus}{
  \newcommand{\var}{x}
  \newcommand{\vartwo}{y}
  \newcommand{\varthree}{z}
  \newcommand{\varfour}{w}

  \newcommand{\tm}{t}
  \newcommand{\tmtwo}{s}
  \newcommand{\tmthree}{u}
  \newcommand{\tmfour}{r}
  \newcommand{\tmfive}{p}
  \newcommand{\tmsix}{q}
  \newcommand{\tmseven}{m}

  \newcommand{\alphaeq}{=_\alpha}

  \newcommand{\esub}[2]{[#1\leftarrow#2]}
  \newcommand\lat{$\lambda$-term}
}

\newnotation{machine-states}{
  \newcommand{\State}{\mathcal{S}}
}

\newnotation{ac-alpha-termgraph}{
  \newcommand{\trx}{\den}
  \newcommand{\trxnp}{\den}
}


==> proofs/line_01.tex <==
% !TEX root = ../main.tex
We discuss \refline{alg_start} together with the first two lines (without numbers on the side) of the procedure $\finish\cdot$.

Every time $\finish \node$ is called in the \textbf{while} loop, either the algorithm fails, or the following state transition occurs: %
\proofTransition{
% State 1
\langle \viviS{1}, {\undS{1}}, {\canS{1}}, \emptyset \rangle
}{
% State 2
\langle \viviS{1}, {\undS{1}}, {\canS{1}} \cup \{(\node,\node)\}, [(\node, \emptyset)] \rangle
}
\proofInvariants{
% Generic considerations
Let us show that the algorithm cannot fail here. It would fail if the canonic of $\node$ was already defined. Let us suppose that $\cS{1}{\node}$ is defined and show that a contradiction follows. Since $\node$ is alive, by \invCanDieLastS{1} and \invCanAliveCanAreDyingS{1} $\cS{1}{\node} \in \RsetS{1}$ but $\RsetS{1}$ is empty, because it is defined starting from $\callstackS{1}$, that is itself empty. Absurd.
Therefore the transition above takes place.

Note that for the canonic relations we have
\begin{itemize}
 \item \emph{canonic}: $(\eqcS{2}) = ({\eqcS{1}} \uplus \{(\node,\node)\})$, because ${\canS{2}} = {\canS{1}} \uplus \{(\node,\node)\}$ and $\cS{1}{\node}=\cundefined$.
 \item \emph{extended canonic}: it is easy to see that $(\eqxS{2}) = ({\eqxS{1}})$ because $\eqxS{}$ is already closed reflexively by definition.
\end{itemize}
Now:
}{
% Preservation of the Interpretation
}{
% Preservation of the Invariants

\begin{enumerate}
 \item % Extended Canonic Relation:
 \proofInvRelations{
 % Congruence
 remember that $(\eqcS{2}) = ({\eqcS{1}} \uplus \{(\node,\node)\})$ and $(\eqxS{2}) = ({\eqxS{1}})$. Because the invariant holds for $\stateS{1}$, we only need to prove it for the new related pair $\node\eqcS{2}\node$ (in fact note that $\node\eqcS{2}\nodetwo$ iff $\node=\nodetwo$):}
 {% Label
    holds because $\node$ has the same label as itself.}
 {% Simulation
    holds because $\eqxS{}$ is reflexive on every node of the term forest.}
 {trivial because $(\eqxS{2}) = ({\eqxS{1}})$.}

 \item % Canonics
 \proofInvCanonics{ we check the invariants for $\node$, because for the other nodes they follow from the hypothesis on $\stateS 1$.
 }{
 % Alive Canonics are Dying
 $\node$ is alive and $\node$ is dying, as required.
 }{
 % Idempotency
 $\cS{2}{\node} = \node$, as required.
 }{
 % Canonics Die Last
 the invariant trivially holds because $\node$ is not dead.
 }{
 % Alive with Canonic is Working
 okay because $\node=\node$ and in fact $\node\not\in\stackS{2}(\node)=\emptyset$. %$\node \in \wclassS{2}{\node}$, as required.
 }

 \item % Alive Nodes:
 \proofInvAlive{
 }{
 % Alive Nodes are Downward Closed
 the set of alive nodes does not change, so the invariant is preserved.
 }{
 % Candidates are Alive
 the candidates and the set of alive nodes do not change, so the invariant is preserved.
 }{
 % Nodes in the Call Stack are Alive
 $\dyingS{2}=\{\node\}$ and $\node$ is alive, as required.
 }
 {nothing new to prove because\\ $\stackS{2}(\node)=\emptyset$.}
 {okay because $\viviS{2}=\viviS{1}$.}

 \item % Working Classes:
 \proofInvClasses{
 % note that there is only one working class, $\wclassS{2}{\node}= \set{\node}$.
 }{
 % Working Nodes have a Dying Canonic
 nothing to prove because $\stackS{2}(\node)=\emptyset$.
 }{
 % Classes are Sets
 true because $\stackS{2}(\node) = \emptyset$.
 }

 \proofInvDying{
 }{
 % Auto-canonic
 $\cS{2}{\node} = \node$, as required.
 }{
 % Calls are on different nodes
 $\dyingS{2} = \set\node$, nothing to prove.
 }{
 % Dying order
 $\dyingS{2} = \set\node$, nothing to prove.
 }

\end{enumerate}
}


==> proofs/line_02.tex <==
% !TEX root = ../main.tex
we discuss \refline{alg6i} together with the first two lines (without numbers on the side) of the procedure $\finish \node$.
There are two cases, either the algorithm fails (because $\cS{1}{\node}$ is already defined) or the program states evolves (when $\cS{1}{\node}$  is undefined).

If the algorithm fails (because $\cS{1}{\node}$ is defined), we show that failure is correct, \ie that $\doppiatilde$ is not a higher-order congruence. Let $\RsetS{1} = [\wcan_1,\ldots,\wcan_k=\wcan]$. Since $\node$ is alive, by \invCanDieLastS{1} and \invCanAliveCanAreDyingS{1} there exists $\wcani$ such that $\cS{1}{\node}=\wcani$, and so $\node \eqcS{1} \wcani$ (by \invClassAutoS{1}).
 We now prove that $\dpathmS{1}$ is cyclic.
 Note that $\node \dpath \wcan$, hence $\wcani \eqcS{1} \node  \dpath \wcan = \wcan_k$, \ie  $\wcani \dpathmS{1} \wcan_k$. Then, by \invPrimDyingOrderS{1} $\wcan_k \dpathmS{1}^* \wcani$ and so $\wcani \dpathmS{1}^+ \wcani$: hence $\doppiatilde$ cannot be a higher-order congruence by \reflemma{prec_irrefl}.

If the call does not fail, the following transition takes place:
\proofTransition{
% State 1
\langle \viviS{1}, \undS{1}, \canS{1}, \callstackS{1} \rangle
}{
% State 2
\langle \viviS{1}, \undS{1}, \canS{1} \cup \{(\node,\node)\}, \callstackS{1} + (\node, \emptyset) \rangle
}
\proofInvariants{
% Generic considerations
If such a transition takes place observe that---as in the case of procedure \procmain above---we have
\begin{itemize}
 \item \emph{canonic}: ${\eqcS{2}} = {\eqcS{1}} \uplus \{(\node,\node)\}$, because ${\canS{2}} = {\canS{1}} \uplus {\{(\node,\node)\}}$.
 \item \emph{extended canonic}: $(\eqxS{2}) = ({\eqxS{1}})$ because $\eqxS{}$ is already closed reflexively by definition.
\end{itemize}

Now:
}{
% Preservation of the Interpretation
}{
% Preservation of the Invariants
mostly as in the case of procedure \procmain, the only minor changes are in the invariants for dying nodes.
\begin{enumerate}
 \item \invbPropQuery: exactly as in the case of procedure \procmain.
 \item \invbCanonics: exactly as in the case of procedure\\ \procmain.
 \item \proofInvAlive{
  }{
  % Alive Nodes are Downward Closed
  the set of alive nodes does not change, so the invariant is preserved.
  }{
  % Candidates are Alive
  the candidates and the set of alive nodes do not change, so the invariant is preserved.
  }{
  % Nodes in the Call Stack are Alive
  the new dying node $\node$ is alive and the old ones are as well by \invDyingAlive
  }
  {follows from \invQueuesAliveS{1}.}
  {okay because $\viviS{2}=\viviS{1}$.}
 \item \invbQueues: it is essentially as in the case of procedure \procmain. The only difference is that now there can be queues other than $\stackS{2}(\node) = \emptyset$, but they are also in $\stateS 1$, so there is nothing else to prove.
 \item % Dying Nodes:
 \proofInvDying{here is the only point where things are slightly different with respect to procedure\\ \procmain, because now there is more than just one dying node. We have $\dyingS{2} = \dyingS{1} \uplus \set\node$ and for the nodes in $\dyingS{1}$ the invariant follows from the invariant for $\stateS{1}$. For $\node$:
 }{
 % Auto-canonic
 $\cS{2}{\node} = \node$, as required.
 }{
 % Calls are on Different Nodes
 by hypothesis $\cS{1}\node$ is undefined (otherwise the algorithm would fail) while by \invClassAutoS{1} all the nodes in $\dyingS{1}$ have their canonical defined, and so $\node \neq \wcani$ for all $\wcani \in \dyingS{1}$.
 }{
 % Primitive Dying Order
 By hypothesis, $\node$ is a parent of $\wcan$, that is, $\node \dpath \wcan$,
 %and $\node\eqcS{2}\node$ and $\wcan\eqcS{2}\wcan$ by \invClassAutoS{2} (already proved).
 and therefore $\node \dpathmS{2} \wcan$.
 }


\end{enumerate}
}


==> proofs/line_09.tex <==
% !TEX root = ../main.tex
The line of the algorithm induces the following transition of states:
\proofTransition{
% State 1
\langle \viviS{1}, \undS{1}, \canS{1}, \callstackS{2} + (\wcan, \emptyset) \rangle
}{
% State 2
\langle \viviS{1}\setminus\{\wcan\}, \undS{1}, \canS{1}, \callstackS{2}\rangle
}
where we know that $\stackS{1}_\wcan$ is empty because that is the condition to exit from the while-cycle before the line under analysis.

Note that many of the notions derived from $\stateS{1}$ and $\stateS{2}$ coincide:
\begin{itemize}
 \item $(\eqcS{1}) = (\eqcS{2})$: because $\canS{1} = \canS{2}$.
 \item $(\eqxS{1}) = (\eqxS{2})$: because $(\eqcS{1}) = (\eqcS{2})$ and ${\undirS{1}}={\undirS{2}}$.
\end{itemize}
Now,
\proofInvariants{
% Generic considerations
}{
% Preservation of the Interpretation
}{
% Preservation of the Invariants

\begin{enumerate}
 \item % Extended Canonic Relation:
 \invbPropQuery:
 immediate, because $(\eqcS{1}) = (\eqcS{2})$ and $(\eqxS{1}) = (\eqxS{2})$.
 \item % Canonics
 \proofInvCanonics{
 }{
 % Alive Canonics are Dying
 trivial because it holds for $\stateS{1}$
 }{
 % Idempotency
 trivial because it holds for $\stateS{1}$
 }{
 % Canonics Die Last
 because it holds for $\stateS{1}$ and $\wcan$ is the only new dead node,
 we only need to prove that for all
 $\node$ s.t. $\canS{1}(\node) = \wcan$ , $\node$ is dead in $\stateS{2}$. If $\node$ was dead in $\stateS{1}$ it is still dead and there is nothing to prove. Otherwise, by \invCanAliveWithCanonicIsWorkingS{1}, either $\node = \wcan$ (and thus it is dead in $\stateS{2}$) or $\node \in \stackS{1}(\wcan) = \emptyset$ (absurd).
 }{
 % Alive with Canonic is Working
 trivial because it holds for $\stateS{1}$
 }

 \item % Alive Nodes:
 \proofInvAlive{
 }{
 % Alive Nodes are Downward Closed
 $\viviS{2} = \viviS{1}\setminus\{\wcan\}$. Therefore we need to prove that all ancestors of $\wcan$ in $\stateS{1}$ are dead. Because of \invAliveDownClosedS{1}, $\mortiS{1}$ is upward closed and therefore it is sufficient to prove that $\wcan$ has no parent in $\viviS{1}$. The property holds because it was established in line $\ref{alg6i}$ and it is preserved in the following lines because the algorithm never changes the term forest and never makes a dead node alive. %\Andrea{salto nel vuoto}
 }{
 % Candidates are Alive
 ${\undirS{1}}={\undirS{2}}$, but $\viviS{2} = \viviS{1}\setminus \set{\wcan}$. Therefore we need to prove that there is no $\node$ such that $\wcan\undirS{}\node$. The property holds because it was established in line $\ref{alg7i}$ and it is preserved in the following lines because:
 \begin{enumerate}
  \item undirected arcs are only added by\\
   \procpush and only to children of alive nodes;
  \item $\wcan$ has no alive parent nodes (and thus cannot participate in new undirected arcs) because the property was established in line $\ref{alg6i}$ (before line $\ref{alg7i}$) and it is preserved in the following lines because the algorithm never changes the term forest and never makes a dead node alive. %\Andrea{salto nel vuoto}
 \end{enumerate}
 }{
 % Nodes in the Call Stack are Alive
 it follows from the invariant for $\stateS 1$, because the only newly dead node $\wcan$ has been removed from the call stack, which contained no duplicates
 because of \invDyingDiffCallsS{1}.
 }  { $\wcan$ is the only node that dies and therefore it is sufficient to show that for all dying node $\wcani$ of $\stateS{2}$, $\wcan \not \in \stackS{2}(\wcani)$. Assume that $\wcan \in \stackS{2}(\wcani)$. By
  \invClassWorkingHaveDyingCanonicS{1}, $\canS{1}(\wcan) = \wcani$.
  Thus by \invDyingAliveS{1} and \invCanAliveWithCanonicIsWorkingS{1} we
  obtain $\wcan = \wcani$, which is absurd because $\wcan$ has been removed
  from the call stack, which contained no duplicates because of
  \invDyingDiffCallsS{1}.
  }%
  { $\wcan$ is the only node that dies, but $\canS{2}(\wcan) = \wcan \neq \cundefined$ by \invClassAutoS{1}. }

 \item \textbf{Queues}: it follows from the invariant for $\stateS 1$, because $\stateS 2$ only lacks one dying node and its queue (the others being preserved).

 \item \textbf{Dying Nodes}: it follows from the invariant for $\stateS 1$, because in $\stateS 2$ there is one dying node less ($\wcan=\wcan_k$) and the others are preserved.


\end{enumerate}
}


==> proofs/line_push.tex <==
% !TEX root = ../main.tex
\mbox{~}

The procedure \procpush is called on \reflineTwo{alg7i}{alg7} of \procfinish. In both cases, we discuss the call to
 \procpush together with the line ``delete undirected edge $(-, \node)$''.

\uline{Note that we carry the proof on the nodes $r$, $s$, and $n$, with the convention that on \refline{alg7i} they stand respectively for $r$, $r$, and $n$.}

In both calls to \procpush, the following facts hold:
\begin{enumerate}
 \item $\wcan$ is the topmost element of $\RsetS{1}$;
 \item $\wcan \eqcS{1} \sthead$ because: on \refline{alg7i} $\wcan \eqcS{1} \wcan$ by \invClassAutoS{1}; on \refline{alg7} $\wcan \eqcS{1} \sthead$ by \invClassAutoS{1} and \invClassWorkingHaveDyingCanonicS{1};
 \item $\wcan \eqxS{1} \node$ because: the item above, and $\sthead \undirS{1} \node$.
 \item $\node \in \viviS{1}$, by \invAliveCandidatesS{1};
 \item $\wcan \in \viviS{1}$, by \invDyingAliveS{1}.
\end{enumerate}

Each call to $\procpush(\stack, r, \node)$ either fails on \reflineTwo{alg_clash}{alg_push_fail}, or it makes the state evolve.
\begin{itemize}
 \item Failure on \refline{alg_clash}: by hypothesis $\wcan \eqxS{1} \node$ and so $\wcan \doppiatilde \node$ (by \pinvpreservation), but they have different labels. Therefore \emph{Label} fails for $\doppiatilde$, which then is not a higher-order congruence.

 \item Failure on \refline{alg_push_fail}: let $\RsetS{1} = [r_1,\ldots,\wcan_k = \wcan]$. By hypothesis $\cS{1}{\node} \neq \wcan = \wcan_k$. Since $\node$ is alive, by \invCanDieLast and \invCanAliveCanAreDyingS{1},
 $\cS{1}{\node}$ is dying, \ie that there is $i$ such that $\cS{1}{\node} = \wcan_i \neq \wcan_k$.
 By \invPrimDyingOrderS{1},  $\wcan_k \dpathmS 1 ^+ \wcani$. Now note that $\cS{1}{\node} = \wcan_i$ implies $\wcan_i \eqxS 1 \node$ (by \invClassAutoS{1}), that together with $\wcan \eqxS{1} \node$ produces $\wcan_i \eqxS 1 \node \eqxS 1 \wcan = \wcan_k \dpathmS 1 ^+ \wcani$,
 that is $\wcan_i \dpathmS 1 ^+ \wcani$, \ie the dying order is cyclic. Therefore $\doppiatilde$ is not a higher-order congruence by \reflemma{prec_irrefl}.
\end{itemize}

If the call does not fail there are two cases:
\begin{itemize}
  \item \emph{$\cS{1}{\node}$ is defined}. Then the only difference between $\stateS{1}$ and $\stateS{2}$ is that ${\undS{2}}={\undS{1}}\setminus\set{(\sthead, \node)}$. But then, since $\cS{1}{\node}=\wcan$, by \invClassAutoS{1}, $\wcan\eqcS{1} \node$, which together with $\wcan \eqcS{1} \sthead$, shows that $\sthead \eqcS{1} \node$. Hence ${\eqxS{1}}={\eqxS{2}}$.
It is easy to see that all invariants are preserved: the only ones worth discussing are \invAliveCandidates{} (which is immediate), and \pinvpreservation{} (because ${\eqxS{1}}={\eqxS{2}}$).

  \item \emph{$\cS{1}{\node}$ is undefined}. Then the following state transition occurs:
\proofTransition{
% State 1
\langle \viviS{1}, \undS{1}, \canS{1}, \callstack + (\wcan, \stackS{1}) \rangle
}{
% State 2
\langle \viviS{1}, {\undS{2}}, \canS{1}\uplus\set{(\node,\wcan)}, \callstack + (\wcan, \stackS{1}\uplus\set{\node})\rangle
}
where $\undS{2}$ depends on whether $\wcan$ has children or not:
\begin{itemize}
 \item if $\wcan$ is a var-node, then $\undS{2}={\undS{1}} \setminus \set{(\sthead, \node)}$. Note that in this case ${\eqxS{1}}={\eqxS{2}}$ since $\sthead \eqcS{2} \node$ (because $\wcan\eqcS{2} \node$ -- from $\cS{2}{\node}=\wcan$ and \invClassAutoS{2} -- and $\wcan \eqcS{1} \sthead$);
 \item otherwise, $\undS{2}={\undS{1}} \setminus \set{(\sthead, \node)} \cup \set{(\wcan_1,\node_1), (\wcan_2,\node_2)}$. In this case ${\eqxS{1}}\subseteq{\eqxS{2}}$ because: ${\eqcS{1}}\subseteq{\eqcS{2}}$, $\undS{1} \setminus \set{(\sthead, \node)} \subseteq \undS{2}$, and $\sthead \eqcS{2} \node$.
\end{itemize}

Note that, because $\undS{\cdot}$ is a multi-relation, $\undS{1} \setminus \{(\sthead,\node)\}$ may still contain occurrences of the pair $(\sthead,\node)$.

\proofInvariants{
% Generic considerations
}{}{
% Preservation of the Invariants
\begin{enumerate}
 \item % Extended Canonic Relation:
 \proofInvRelations{
  Recall that $(\eqcS{1}) \neq (\eqcS{2})$ because $\canS{2} = \canS{1} \uplus \set{(\node,\wcan)}$.
 }{ % Label
Let $\nodetwo\eqcS{2}\nodetwo'$: we need to prove that $\nodetwo$ and $\nodetwo'$ have the same label. If $\nodetwo\eqcS{1}\nodetwo'$, the requirement follows from \invExtCongS{1}. Assume then $\nodetwo\not\eqcS{1}\nodetwo'$: this means that necessarily  $\wcan = \cS{2}{\nodetwo} = \cS{2}{\nodetwo'}$.

   Note that either $\nodetwo$ or $\nodetwo'$ is $\node$, because otherwise $\nodetwo\eqcS{1}\nodetwo'$; hence three cases:
   \begin{itemize}
    \item $\nodetwo=\nodetwo'=\node$: trivial, because $\node$ has the same label as itself;
    \item $\nodetwo = \node$ and $\nodetwo' \neq \node$.
    $\cS{1}{\nodetwo'}=\wcan$ implies $\nodetwo'\eqcS{1}\wcan$ (by \invClassAutoS{1}), and implies by \invExtCongS{1} that $\nodetwo'$ and $\wcan$ have the same label. In order to conclude, it suffices to show that $\wcan$ and $\nodetwo=\node$ have the same label: This is the case because of the check on \refline{alg_clash}.
    \item $\nodetwo \neq \node$ and $\nodetwo' = \node$: symmetric to the case above.
   \end{itemize}
 }{ % Simulation
Let $\nodetwo\eqcS{2}\nodetwo'$. If $\nodetwo\eqcS{1}\nodetwo'$, the requirement follows from \invExtNecS{1} because ${\eqxS{1}} \subseteq {\eqxS{2}}$. Assume then $\nodetwo\not\eqcS{1}\nodetwo'$: this means that necessarily  $\wcan = \cS{2}{\nodetwo} = \cS{2}{\nodetwo'}$.

   Recall: we need to prove that if $\nodetwo\dpath_i\nodetwo_i$ then $\nodetwo'\dpath_i\nodetwo_i'$ and $\nodetwo_i \eqxS{2} \nodetwo_i'$. Note that either $\nodetwo$ or $\nodetwo'$ is $\node$, because otherwise $\nodetwo\eqcS{1}\nodetwo'$; hence three cases:
   \begin{itemize}
    \item $\nodetwo=\nodetwo'=\node$: trivial, because if $\node\dpath_i\node_i$ then $\node\dpath_i\node_i$ and $\node_i \eqxS{2} \node_i$ (because $\eqxS{2}$ is reflexive);
    \item $\nodetwo = \node$ and $\nodetwo' \neq \node$. Suppose $\nodetwo\dpath_i\nodetwo_i=\node_i$: by the requirement Label proved above, $\nodetwo$ and $\nodetwo'$ have the same label (because $\nodetwo\eqcS{2}\nodetwo'$), hence $\nodetwo'\dpath_i\nodetwo_i'$ for some $\nodetwo_i'$.

    $\cS{1}{\nodetwo'}=\wcan$ implies $\nodetwo'\eqcS{1}\wcan$ (by \invClassAutoS{1}), and implies by \invExtNecS{1} that $\wcan\dpath_i\wcan_i$ and $\nodetwo_i' \eqxS{1} \wcan_i$. Because $\nodetwo_i = \node_i \undirS{2} \wcan_i$ and ${\eqxS{1}}\subseteq{\eqxS{2}}$, we conclude with $\nodetwo_i \eqxS{2} \nodetwo_i'$.

    \item $\nodetwo \neq \node$ and $\nodetwo' = \node$: (almost) symmetric to the case above.
   \end{itemize}
 }
 {We have ${\eqxS{1}} \subseteq {\eqxS{2}}$. Therefore we just need to show the second inclusion of the invariant.

 Note that $\doppiatilde$ contains $\eqxS{2}$ iff it contains $\eqxS{1}$ and it contains $\set{(\wcan_1, \node_1), (\wcan_2, \node_2)}$. The first follows from \pinvpreservation{} for $\stateS{1}$. The second follows from $\wcan \doppiatilde \node$ by definition of $\doppiatilde$.
}

 \item % Canonics
 \proofInvCanonics{ We only have to consider the new case $\cS{2}\node = \wcan$, for which:
 }{
 % Alive Canonics are Dying
 $\wcan$ is dying in $\stateS 2$ because it is so in $\stateS 1$.
 }{
 % Idempotency
 $\cS{2}{\wcan} = \cS{1}{\wcan} = \wcan$ by \invClassAutoS 1.
 }{
 % Canonics Die Last
 $\wcan$ is alive so the hypothesis is false and the invariant trivially holds.
 }{
 % Alive with Canonic is Working
 $\wcan$ is dying and $\node\neq\wcan$ (because $\cS{1}{\wcan}=\wcan$ by \invClassAutoS{1}, while $\cS{1}{\node}=\cundefined$) and $\node\in \stackS{2}(\wcan)$, as required.
 }

 \item % Alive Nodes:
 \proofInvAlive{
 }{
 % Alive Nodes are Downward Closed
 the set of alive nodes does not change.
 }{
 % Candidates are Alive
 The new edges involve children of $\wcan$ and $\node$. We already proved that $\wcan$ and $\node$ are alive. By \invAliveDownClosedS{1}, $\set{\wcani,\node_i} \subseteq \viviS{1}$ and we conclude.
 }{
 % Nodes in the Call Stack are Alive
 the set of dying nodes does not change.
 }{the only new node in the queues is $\node$, that we already proved to be alive.
 }{immediate by \invDeadReprS{1}.}

 \item % Working Classes:
 \proofInvClasses{ We only have to consider the case $\stackS{2}_{\wcan} = \stackS{1}_{\wcan} \uplus \set\node$, for which:
 }{
 % Working Nodes have a Dying Canonic
 $\cS{2}\node = \wcan$ as required.
 }{
 % Classes are Sets
 $\node$ is distinct from every other node $\nodetwo \in \stackS{1}(\wcan)$ because by \invClassWorkingHaveDyingCanonicS 1, $\nodetwo$ has the canonic defined in $\stateS{1}$ while $\node$ does not. The nodes in $\stackS{1}_{\wcan}$ are pairwise distinct because the invariant holds on $\stateS{1}$.
 }

 \item \proofInvDying{}
  {preserved.}
  {the set of dying nodes does not change.}
  {the set of dying nodes does not change, and ${\eqxS{1}}\subseteq{\eqxS{2}}$.}

\end{enumerate}
\end{itemize}


}


==> proofs/preservation_of_good_invariants.tex <==
% !TEX root = ../main.tex
\begin{proof}[Proof of \refthm{huge}]\label{proof:of-huge}
 We discuss separately each line of the algorithm, one procedure at a time.
 But first note the following, which hold after any successful state transition:
 \begin{itemize}
  \item ${\canS{1}}\subseteq{\canS{2}}$, because canonical pointers are never deleted;
  \item $({\eqcS{1}})\subseteq(\eqcS{2})$ for the same reason;
  % \item ${(\dpathmS{1})}\subseteq{(\dpathmS{2})}$ for the same reason, and because directed edges are never deleted;
  \item $\viviS{2} \subseteq \viviS{1}$ because nodes are never marked alive;
 \end{itemize}

For reasons of clarity, we are going to drop the term forest from (refined) states, denoting $\pstate=\stateS{1}=\langle \viviS{1}, \undS{1}, \canS{1}, \callstackS{1} \rangle$ and $\pstate'=\stateS{2}=\langle \viviS{2}, \undS{2}, \canS{2}, \callstackS{2} \rangle$.

\vspace{0.2in}

 \paragraph*{Procedure \procmain}~
 \begin{itemize}
  \item[(\ref{alg_start})] \input{\proofspath/line_01}
 \end{itemize}
 \paragraph*{Procedure \procfinish}~
 \begin{itemize}
  \item[(\ref{alg6i})] \input{\proofspath/line_02}
  \item[(\ref{alg7i})] See procedure \procpush below.

  \item[(\ref{alg6})] Identical to the proof for \refline{alg6i}, except for:
   \begin{itemize}
    \item in that for \refline{alg6i} to deal with failure we conclude
      $\node \dpathmS{1} \wcan$ from $\node \dpath \wcan$. Here we
      reach the same conclusion from $\node \dpath \sthead \eqxS{1} \wcan $;
    \item similarly, \invPrimDyingOrder for $\node$ holds because $\node = \wcan_{k+1} \dpath \sthead_k = s \eqcS{} \wcan_{k}$ (while for \refline{alg6i} it holds because $\node = \wcan_{k+1} \dpath \wcan_k = \wcan$).
   \end{itemize}

  \item[(\ref{alg7})]  See procedure \procpush below.
  \item[(\ref{alg11})] \input{\proofspath/vars_and_s_dies}
  \item[(\ref{alg12})] \input{\proofspath/line_09}

 \end{itemize}

 \paragraph*{Procedure \procpush}

 \input{\proofspath/line_push}

\end{proof}


==> proofs/termination_in_linear_time.tex <==
% !TEX root = ../main.tex
\begin{proof}
First note that if $\pstate'=\failure$, then $\size{\pstate}>0$ by \refrem{size-good-pos}.

Now we discuss separately each procedure of Algorithm~\ref{alg:sharing-check}, similarly as in the proof of \refthm{huge} on page~\pageref{proof:of-huge}.

\paragraph*{Procedure \procmain:}

% \begin{itemize}
%  \item[(\ref{alg_start})]
we discuss \refline{alg_start} together with the first two lines (without numbers on the side) of the procedure $\finish\node$. In case it does not fail, the state $\pstate'$ after the call differs from $\pstate$ by having one more canonical representative set. Therefore $\size{\pstate'} = \size{\pstate} - 2 < \size{\pstate}$.

 % \item[(\ref{alg:check_var_nodes}-\ref{alg:propagate.failDue})] The \textbf{while} is executed at most once by the algorithm, it clearly terminates, and its body (which runs in constant time) is executed a number of times $\leq\nodes$, hence linear in the numbers of nodes of the term forest. \Andrea{non mi sembra questo il posto giusto per questo ragionamento, forse va nella prova del corollario qui sopra?}
% \end{itemize}

\paragraph*{Procedure \procfinish:} we discuss separately each line of the procedure.
\begin{itemize}
 \item[(\ref{alg6i})] Exactly like the case of the loop on \refline{alg_start} of \procmain.

 \item[(\ref{alg7i})] See procedure \procpush below.

 \item[(\ref{alg6})] Exactly like the case of the loop on \refline{alg_start} of \procmain.

 \item[(\ref{alg7})] See procedure \procpush below.

 \item[(\ref{alg11})] $\pstate'$ differs from $\pstate$ by having one more dead node: hence $\size{\pstate'} = \size{\pstate} - 1 < \size{\pstate}$.

 \item[(\ref{alg12})] $\pstate'$ differs from $\pstate$ by having one more dead node: hence $\size{\pstate'} = \size{\pstate} - 1 < \size{\pstate}$.

\end{itemize}

\noindent Procedure \procpush: it is called on \reflineTwo{alg7i}{alg7} of \procfinish. In both cases, we discuss the call to
 \procpush together with the unnumbered line ``delete undirected edge $(-, \node)$''.
 There are three possible outcomes:
 \begin{itemize}
  \item the case of failure was already discussed above;
  \item if $\cS{}{\node}=\wcan$, then $\pstate'$ differs by $\pstate$ only for having one undirected arcs less, hence $\size{\pstate'} = \size{\pstate} - 1 < \size{\pstate}$;
  \item if $\cS{}{\node}=\cundefined$, then we have one undirected arc less, one canonical assignment more, and $x$ undirected arcs more where $x \leq 2$.
  Hence
  $\size{\pstate'} = \size{\pstate} - 1 - 2\,\, + x < \size{\pstate}$.
 \end{itemize}

\end{proof}


==> proofs/vars_and_s_dies.tex <==
% !TEX root = ../main.tex

We discuss \refline{alg11} and the following one without a number.

The following state transition occurs: %
\proofTransition{
% State 1
\langle \viviS{1}, {\undS{1}}, {\canS{1}}, \callstackS{1} \rangle
}{
% State 2
\langle \viviS{1}\setminus \{\sthead\}, {\undS{1}}, {\canS{1}}, \callstackS{2} \rangle
}
\proofInvariants{
% Generic considerations
The only difference between $\callstackS{1}$ and $\callstackS{2}$ is that $\stackS{1}(\wcan)=\stackS{2}(\wcan)\uplus\set{\sthead}$. Therefore clearly $(\eqcS{2}) = (\eqcS{1})$ and $(\eqxS{2}) = (\eqxS{1})$.
Moreover $\sthead \neq \wcan$ by \invCanAliveWithCanonicIsWorkingS{1} because
$\sthead \in \stackS{1}(\wcan)$ and
$s \in \viviS{1}$ (by \invQueuesAliveS{1}).

Now:
}{
% Preservation of the Interpretation
}{
% Preservation of the Invariants

\begin{enumerate}
 \item % Extended Canonic Relation:
 \proofInvRelations{
 % Congruence
 }{ % Label
 trivial, because $(\eqcS{2}) = (\eqcS{1})$ and $(\eqxS{2}) = (\eqxS{1})$.
 }{ % Simulation
 trivial, because $(\eqcS{2}) = (\eqcS{1})$ and $(\eqxS{2}) = (\eqxS{1})$.
 }
 { immediate because ${\undirS{1}}={\undirS{2}}$ and ${\eqcS{1}}={\eqcS{2}}$. }

 \item \textbf{Canonics}: the canonical assignment does not change (\ie $\canS 1 = \canS 2$) and the only node that is killed is $\sthead$. Therefore all invariants are trivially preserved but \invCanDieLast that requires to prove that there is no alive node $\nodetwo$ such that $\can(\nodetwo) = \sthead$. By absurdum, if such a node existed by \invCanIdempS{1} one would have $\can(\sthead) = \sthead$ whereas $\can(\sthead) = \wcan$ by \invClassWorkingHaveDyingCanonic. Therefore it would be the case $\sthead = \wcan$ that is absurd (we already proved $\sthead \neq \wcan$).

 \item % Alive Nodes:
 \proofInvAlive{
 }{
 % Alive Nodes are Downward Closed
 $\viviS{2} = \viviS{1}\setminus\set\sthead$. Therefore we need to prove that all ancestors of $\sthead$ in $\stateS{1}$ are dead. Because of \invAliveDownClosedS{1}, $\mortiS{1}$ is upward closed and therefore it is sufficient to prove that $\sthead$ has no parent in $\viviS{1}$. Similarly to what we will discuss on \refline{alg12}, this property was established on \refline{alg6} and it is preserved in the following lines because the algorithm never changes the term forest, and never makes a dead node alive.
 }{
 % Candidates are Alive
 again, similar to what we will discuss for \refline{alg12}.
 }{
 % Nodes in the Call Stack are Alive
 it follows from the property for $\stateS{1}$, because the dying set does not change and we now prove that the only node $\sthead$ that dies was not dying in $\stateS{1}$. Indeed $\cS{1}{\sthead} = \wcan$ by \invClassWorkingHaveDyingCanonic and for every $\wcani$ in the dying set $\cS{1}{\wcani} = \wcani$ by \invClassAuto. Therefore $\sthead$ could only be equal to the dying node $\wcan$, but we already proved $\sthead \neq \wcan$.
 }
 { $\sthead$ is the only node that dies and therefore it is sufficient to show that for every dying node $\wcani$, $\sthead \not \in \stackS{2}(\wcani)$.
By \invClassWorkingHaveDyingCanonicS{1} and \invDyingDiffCallsS{1}, all queues
have distinct elements, $\sthead \in \stackS{1}(\wcani)$ by \invClassWorkingHaveDyingCanonicS{1} and thus $\sthead$ does not belong to the other queues. Therefore it belongs to no queue in $\stateS{2}$ because it is removed from $\stackS{2}(\wcan)$.
}
 { $\sthead$ is the only node that dies, but $\cS{1}{\sthead} = \wcan \neq \cundefined$ by \invClassWorkingHaveDyingCanonicS{1}. }

 \item \textbf{Queues}: dying nodes are preserved and all queues stay the same but for $\stack(\wcan)$, that shrinks ($\stackS{1}(\wcan) = \stackS{2}(\wcan) \uplus \set{\sthead}$). Then the invariants are trivially preserved.

 \item \textbf{Dying Nodes}: the set of dying nodes does not change and so the invariants are trivially preserved.


\end{enumerate}
}


==> related.tex <==
\section{Related works}

We are aware of other two papers that consider the problem of sharing equivalence in presence of binders. The first one is ~\cite{DBLP:conf/rta/AccattoliL12} % Accatoli and Dal Lago
where a quadratic algorithm is presented. The second one is ~\cite{DBLP:conf/icfp/GrabmayerR14} where the $\lambda$-calculus considered has recursive \texttt{let} definitions. Therefore the problem there is much harder because terms are to be compared not only up to $\alpha$-equivalence, but also up to infinite unsharing. The algorithm proposed performs a complex encoding of the terms in first-order graphs where additional nodes are introduced to record information about scopes. Finally, a variant of the Hopcroft-Karp~\cite{hoka71} algorithm to test equivalence of deterministic finite automata is employed. The latter algorithm has quasi-linear complexity, i.e. it is in $O(n\cdot \alpha(n))$ where $\alpha(\cdot)$ is the inverse of the Ackermann function. However, when the reduction to first order graphs is considered, the final complexity of Grabmayer and Rochel is $O(n^2 \cdot \alpha(n)$.

Obtaining directly a quasi linear time for sharing equivalence from the Hopcroft-Karp algorithm is easy, but it has never been spelled out. Intuitively one can see the nodes of a term forest as states of a DFA and arcs $\node \dpath_i \nodetwo$ as transitions labelled by $i$. Moreover, an arc is put between variables and their binders, representing transitions labelled by a special symbol. It then remains to determine if the pairs of nodes in the query represent equivalent automata states. The algorithm of Hopcroft-Karp just needs to be slightly modified by checking also that equivalent nodes have the same label and by accepting equivalent free variable nodes only if they are equal (the automata have no accepting states). The key result of our paper that links $\alpha$-equivalence with well-scoped queries is still necessary to understand sharing equivalence in term of $\alpha$-equivalence problems. Moreover, \refthm{soundness} can still be exploited to obtain a different algorithm by splitting the construction of the spreaded query from the check that it is a \hocongruence: when the query is scoped, one can just drop from the automata construction the arcs introduced by the binders and perform the $\lambda$ check if the Hopcroft-Karp algorithm succeds. Which variant runs faster in practice is to be understood.

It is likely that a quasi-linear algorithm based on Hopcroft-Karp can run faster in practice than our linear algorithm. The main interest in our proof of linearity is then theoretical.

The problem of sharing equivalence has been mostly neglected also for first-order languages, with the notable exception of~\cite{Martelli:1977:TPS:1624435.1624556} where Martelli and Montanari develop a linear algorithm to unify first-order terms encoded using the Boyer-Moore technique~\cite{boyer1972sharing}, which exploits sharing. While the source of sharing in that paper comes from previous unification steps in resolution proofs --- we are essentialy in the domain of logic programming --- our source of sharing is to perform efficiently reduction in the $\lambda$-calculus --- the domain of functional programming. That algorithm by Martelli and Montanari only works for first-order terms. The one that became famous as the Martelli and Montanari unification algorithm is a different one that is explonential when applied to shared terms.

The problem of sharing equivalence in presence of binders can be reduced to known ones in two different ways.
\begin{enumerate}
 \item \emph{Reduction to (nominal/pattern) unification}: a term forest can be encoded in linear time as an unification problem by replacing, before reading-back the term, all non-variable nodes that have at least two parents with an unification variable and then adding an equation to force unification of the variable with the read-back of the corresponding term. For example, the sharing equality problem between the maximally shared form of the term $(\lambda x.(x x)(x x))(\lambda x.(x x)(x x))$ and itself becomes the system of equations $\{XX=XX, X=(\lambda x.YY), Y=(xx)\}$ where $x$ is allowed to occur in $Y$. The system of equations can be faithfully represented with minor syntactic changes both as a pattern unification problem or as a nominal unification problem. The reduction to nominal unification yields a quadratic algorithm, because the two best known algorithms for it have both quadratic complexity~\cite{Calves:2010:FNL:2008282.2008297,4030}. On the other hand the reduction to pattern unification yields an alternative linear algorithm because of a linear algorithm by Qian~\cite{10.1007/3-540-56610-4_78}. We have not investigated the relation between the two linear algorithms, but we note that Qian algorithm is very involved, requires a lot more code and more data structures and the overall algorithm would surely have higher computational constants than ours. Indeed, according to~\cite{4030}, ``it is really difficult to obtain a practical algorithm from the proof described in~\cite{10.1007/3-540-56610-4_78}''.
 \item \emph{Sharing equality as a special case of nominal/pattern unification/matching}: $\alpha$-equality is a special case of pattern unification and unificaition and $\lambda$-terms are nominal/pattern terms where unification variables and permutations do not occur. Therefore any algorithm for nominal/patter unification/matching that works on terms represented as DAGs would solve our problem as well. However, the papers in the literature either work on first-order DAGs~\cite{PATERSON1978158}, or they have non-linear complexity~\cite{Calves:2010:FNL:2008282.2008297,calvs:LIPIcs:2013:4059} even when fed with plain $\lambda$-terms as DAGs, or they only work when the terms have not sharing (but for variables)~\cite{10.1007/3-540-56610-4_78}, or they are based (like~\cite{CALVES2010283}) on Martelli-Montanari \cite{Martelli:1982:EUA:357162.357169} that is not linear in the size of the terms when the terms are represented as DAGs. Actually, it is an interesting observation that the high-level explanation of Paterson-Wegman algorithm in Martelli-Montanari style, at the base of many recent algorithms, misses one important feature of the original algorithm: that of taking in input DAGs and being linear on them.
\end{enumerate}

In~\cite{calvs:LIPIcs:2013:4059} an abstract algorithm to solve nominal unification problems, based on Wagner-Paterson and subsuming the two best known algorithms is presented. The key idea is to enrich Wagner-Paterson with an additional data structure, called \emph{modality}, that records freshness constraints and identification/swapping of variables. In our restricted case, only the identification of variables is required and the modality is just a representation of the $\nameset$ in $\convren$. Managing the modality has a cost: the two best algorithms do that in different ways, but always with a linear overhead per operation, yielding the final quadratic complexity. Our contribution can be seen as showing that no explicit modality data structure is required at all --- and thus no overhead at all --- to check sharing equality: the information about identification of (bound) variables is already encoded by the canonical pointers of their binders.

Wagner-Paterson algorithm, and thus ours as well, requires all nodes to point to their parents. The DAGs used for efficient reduction of $\lambda$-terms miss these backward-pointers. De Champeaux gave an algorithm to add them in linear time~\cite{DECHAMPEAUX198679}.

Finally, the fact that our algorithm first uses Wagner-Paterson algorithm considering all variables equal and only after it checks that the computed relation is a $\lambda$-sharing equality is a direct application of the ``first-order nominal link'' of~\cite{Calves:2010:FNL:2008282.2008297}.


==> xstring.tex <==
%  __________________________________________________
% |                                                  |
% |                                                  |
% |                   xstring v1.7c                  |
% |                                                  |
% |                  13 octobre 2013                 |
% |                                                  |
% |__________________________________________________|
%
% This is xtring.tex
%
% "xstring" package consists of the 7 following files:
%   xstring.tex (this file)
%   xstring.sty
%   README
%   xstring_doc_fr.tex, xstring_doc_fr.pdf (manual in french)
%   xstring_doc_en.tex, xstring_doc_en.pdf (manual in english)
%
% Christian Tellechea 2008-2013
% email : unbonpetit@gmail.com
% -------------------------------------------------------------------
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%
%     http://www.latex-project.org/lppl.txt
%
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% -------------------------------------------------------------------
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Christian Tellechea
% -------------------------------------------------------------------
\def\xstringversion     {1.7c}
\def\xstringdate        {2013/10/13}
\def\xstringfrenchdate  {13 octobre 2013}
\def\xstringenglishdate {13 october 2013}
\edef\CurrentAtCatcode  {\the\catcode`\@}
\catcode`\@=11
\newwrite\@xs@message% canal pour les messages
\newcount\integerpart
\newcount\decimalpart% compteurs utilis\'es par xstring

\expandafter\ifx\csname @latexerr\endcsname\relax% on n'utilise pas LaTeX ?
	\immediate\write\m@ne{Package: xstring \xstringdate\space\space v\xstringversion\space\space String manipulations}%
	\long\def\@firstoftwo#1#2{#1}
	\long\def\@secondoftwo#1#2{#2}
	\long\def\@gobble#1{}
	\long\def\@ifnextchar#1#2#3{%
		\let\reserved@d=#1%
		\def\reserved@a{#2}%
		\def\reserved@b{#3}%
		\futurelet\@let@arg\@ifnch}
	\def\@ifnch{%
		\ifx\@let@arg\@sptoken
			\let\reserved@c\@xifnch
		\else
			\ifx\@let@arg\reserved@d
				\let\reserved@c\reserved@a
			\else
				\let\reserved@c\reserved@b
			\fi
		\fi
		\reserved@c}
	\def\:{\let\@sptoken= } \:
	\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@arg\@ifnch}
	\def\@ifstar#1{\@ifnextchar *{\@firstoftwo{#1}}}
	\long\def\@testopt#1#2{\@ifnextchar[{#1}{#1[{#2}]}}
	\def\@empty{}
\fi% fin des d\'efinitions LaTeX

\long\def\@xs@ifempty#1{%
	\expandafter\ifx\expandafter\relax\detokenize{#1}\relax
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}
% Ouvre un groupe o\`u les catcodes sont \`a 12 et \`a 10 pour les espaces
% ensuite, appelle \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\@xs@MakeVerb{% lit 1 argument et le transforme en verb
	\begingroup% groupe o\`u les catcodes sont \`a 12 pour la lecture suivante
		\def\do##1{\catcode`##112\relax}%
		\dospecials% on entre dans le mode verb
		\obeyspaces% et on tient compte des espaces
		\@xs@ReadVerb% et on va lire l'argument
}

% D\'efinit \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\setverbdelim#1{% d\'efinit quel est le d\'elimiteur de verb
	\expandafter\@xs@ifempty\expandafter{\@gobble#1}%
		\relax
		{\begingroup
			\newlinechar`\^^J%
			\immediate\write\@xs@message
			{Package xstring Warning: verb delimiter is not a single token on input line \the\inputlineno^^J}%
		\endgroup
		}%
	\def\@xs@ReadVerb##1#1##2#1{% lit ##2 qui est entre les d\'elimiteurs de verb
		\endgroup% on ferme le groupe
		\@xs@afterreadverb{##2}}% on appelle l'ex\'ecution de fin
}

% Assigne l'argument entre d\'elimiteur verb dans la sc #1' +
\def\verbtocs#1{%
	\def\@xs@afterreadverb##1{\def#1{##1}}%
	\@xs@MakeVerb
}

\begingroup
	\catcode\z@3 \def\@xs@twochars{^^00}%
	\catcode\z@7 \xdef\@xs@twochars{\@xs@twochars^^00}%
\endgroup

\edef\@xs@reserved@A{\long\def\noexpand\@xs@AssignResult##1\@xs@twochars}

\@xs@reserved@A#2{\endgroup\expandafter\def\expandafter#2\expandafter{\@gobble#1}}

\def\tokenize#1#2{%
	\begingroup
		\@xs@def\@xs@reserved@A{#2}% on d\'eveloppe en accord avec \fullexpandarg ou \noexpandarg
		\everyeof\expandafter{\@xs@twochars#1}% met "^^@^^@#1" \`a la fin du fichier virtuel
		\endlinechar\m@ne
		\expandafter\@xs@AssignResult\scantokens\expandafter{\expandafter\relax\@xs@reserved@A}% on fait l'assignation
}%

% Macro tr\`es simple qui assigne ou affiche le r\'esultat, selon la pr\'esence
% ou non de #2 qui est l'argument optionnel venant en derni\`ere position des macros
\long\def\@xs@ReturnResult#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#2}%
		\@xs@argument@A
		{\let#2\@xs@argument@A}%
}

\def\@xs@ldef{\long\def}

\def\@xs@ledef{\long\edef}

% Pas d'expansion des arguments
\def\normalexpandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter{##1}}}
\let\noexpandarg\normalexpandarg% synonyme

% 1-d\'eveloppement du premier token des arguments
\def\expandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter\expandafter\expandafter{##1}}%
}

% D\'eveloppement maximum des arguments
\def\fullexpandarg{%
	\let\@xs@def\@xs@ledef% on d\'efinit\@xs@call avec \edef
	\def\@xs@expand##1{##1}% et on neutralise \@xs@expand
}

\def\saveexpandmode{\let\@xs@saved@def\@xs@defarg\let\@xs@saved@expand\@xs@expand}

\def\restoreexpandmode{\let\@xs@defarg\@xs@saved@def\let\@xs@expand\@xs@saved@expand}

% Macro interne renvoyant #2 si son argument commence par une accolade ouvrante "{"
% et #3 sinon (Ulrich Diez sur comp.text.tex)
\long\def\@xs@ifbeginwithbrace#1{%
	\csname @%
		\expandafter\@gobble\string{%
		\expandafter\@gobble\expandafter{\expandafter{\string#1}%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@firstoftwo
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter{\expandafter\string\expandafter}\string}%
		\expandafter\@gobble\string}%
		\@secondoftwo{first}{second}oftwo%
	\endcsname
}

% Cette macro interne prend la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@returnfirstsyntaxunit#1#2{%
	\def\@xs@groupfound{\expandafter\def\expandafter#2\expandafter{\expandafter{#2}}\@xs@gobbleall}% on met #2 dans des accolades et on finit
	\long\def\@xs@assignfirsttok##1##2\@xs@nil{\let\@xs@toks0\def#2{##1}}%
	\def\@xs@testfirsttok{%
		\let\@xs@next\@xs@assignfirsttok
		\ifx\@xs@toks\bgroup
			\expandafter\@xs@ifbeginwithbrace\expandafter{\@xs@argument}{\def\@xs@next{\afterassignment\@xs@groupfound\def#2}}{}%
		\fi
		\@xs@next}%
	\def\@xs@argument{#1}%
	\edef\@xs@next{\expandafter\@xs@beforespace\detokenize{#1} \@xs@nil}% #1 commence par un espace ?
	\ifx\@xs@next\@empty
		\def\@xs@next{\expandafter\ifx\expandafter\@empty\detokenize\expandafter{\@xs@argument}\@empty\let#2\@empty\else\def#2{ }\let\@xs@toks0\fi}%
	\else
		\def\@xs@next{\expandafter\futurelet\expandafter\@xs@toks\expandafter\@xs@testfirsttok\@xs@argument\@xs@nil}%
	\fi
	\@xs@next
}

% Cette macro interne enl\`eve la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@testsecondtoken#1\@xs@nil{\@xs@ifbeginwithbrace{#1}}

\long\def\@xs@gobblespacebeforebrace#1#{}% supprime tout ce qui est avant la 1ere accolade ouvrante

\long\def\@xs@removefirstsyntaxunit#1#2{%
	\def\@xs@argument{#1}%
	\expandafter\expandafter\expandafter\ifx\expandafter\expandafter\expandafter\@empty\expandafter\@xs@beforespace\detokenize\expandafter{\@xs@argument} \@xs@nil\@empty% #1 commence par un espace ?
		\expandafter\@xs@ifempty\expandafter{\@xs@argument}%
			{\let#2\@empty}
			{\afterassignment\@xs@testsecondtoken% après avoir mangé le 1er token, on va tester si la suite commence par «{»
			\expandafter\let\expandafter\@xs@secontoken\expandafter=\expandafter\@sptoken\@xs@argument\@xs@@nil\@xs@nil% on mange le 1er token et on rajoute \@xs@@nil à la fin pour éviter de perdre les accolades du groupe
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@gobblespacebeforebrace\@xs@argument}}%
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@behindspace\@xs@argument\@xs@nil}}%
			}%
	\else
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
		\expandafter\expandafter\expandafter{\expandafter\@gobble\@xs@argument}%
	\fi
}

% Macros \`a arguments d\'elimit\'es pour les macros ci dessus
\long\def\@xs@beforespace#1 #2\@xs@nil{#1}

\long\def\@xs@behindspace#1 #2\@xs@nil{#2}

\long\def\@xs@returnfirstsyntaxunit@ii#1#2\@xs@nil{#1}

\long\def\@xs@gobbleall#1\@xs@nil{}

% Cette macro interne est utilis\'ee dans les macros \'etoil\'ees pour :
% 1) d\'evelopper l'argument selon qu'on a choisit \fullexpandarg
%    ou \normalexpandarg, et ceci \`a l'aide de la macro \@xs@def
% 2) Ensuite, on d\'etokenize ce d\'eveloppement de façon n'avoir plus que
%    des catcodes de 10 pour les espaces et 12 pour le reste.
\long\def\@xs@expand@and@detokenize#1#2{%
	\long\def#1{#2}%
	\expandafter\edef\expandafter#1\expandafter{\@xs@expand#1}% on d\'eveloppe #2 selon le mode de d\'eveloppement
	\long\edef#1{\detokenize\expandafter{#1}}% puis on d\'etokenize et on assigne \`a #1
}

\long\def\@xs@expand@and@assign#1#2{\@xs@def#1{#2}}% on d\'eveloppe #2 selon \fullexpandarg ou \normalexpandarg

\long\def\@xs@edefaddtomacro#1#2{\edef#1{\unexpanded\expandafter{#1}#2}}

\long\def\@xs@addtomacro#1#2{\expandafter\def\expandafter#1\expandafter{#1#2}}

\def\@xs@argstring{0########1########2########3########4########5########6########7########8########9}

% \@xs@DefArg{3} met dans la sc \@xs@myarg les tokens "####1####2####3"
\def\@xs@DefArg#1{\def\@xs@defarg0##1#1##2\@xs@nil{\def\@xs@myarg{##1#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@DefArg@{3} met dans la sc \@xs@myarg les tokens "[####1]####2####3####4"
\def\@xs@DefArg@#1{\expandafter\@xs@defarg@\expandafter{\number\numexpr#1+1}}

\def\@xs@defarg@#1{\def\@xs@defarg0##11##2#1##3\@xs@nil{\def\@xs@myarg{[##11]##2#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@OneArg{3} met dans la sc \@xs@myarg les tokens "####3"
\def\@xs@OneArg#1{\expandafter\@xs@onearg\expandafter{\number\numexpr#1-1}{#1}}

\def\@xs@onearg#1#2{\def\@xs@defarg##1#1##2#2##3\@xs@nil{\def\@xs@myarg{##2#2}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% #1 : num\'ero du 1er argument; #2 : nombre de lignes; #3 argument optionnel; #4 : dernier num\'ero de l'argument devant être d\'etokenis\'e si \'etoile
\def\@xs@BuildLines#1#2#3#4{%
	\let\@xs@newlines\@empty
	\let\@xs@newargs\@empty
	\def\@xs@buildlines##1{%
		\expandafter\@xs@OneArg\expandafter{\number\numexpr##1+#1-1}%
		\edef\@xs@reserved@B{\noexpand\@xs@expand\csname @xs@arg@\romannumeral\numexpr##1\endcsname}%
		\ifnum##1=\@ne% si c'est le premier argument
			\@xs@ifempty{#3}%
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
				\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
				}% et s'il y a un argument optionnel alors, on met des crochets
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter[\@xs@reserved@B]}%
				\def\@xs@reserved@B{@xs@def}% ne pas d\'etok\'eniser l'argument optionnel grace au \@xs@def
				}
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
			\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
		\fi
		\edef\@xs@newlines{\unexpanded\expandafter{\@xs@newlines}\expandafter\noexpand\csname\@xs@reserved@B\endcsname\expandafter\noexpand\csname @xs@arg@\romannumeral\numexpr##1\endcsname{\@xs@myarg}}%
		\ifnum##1<#2\relax
			\def\@xs@next{\expandafter\@xs@buildlines\expandafter{\number\numexpr##1+1}}%
			\expandafter\@xs@next
		\fi}%
	\@xs@buildlines\@ne
}

\def\@xs@newmacro{%
	\@ifstar
		{\let\@xs@reserved@D\@empty\@xs@newmacro@}
		{\let\@xs@reserved@D\relax\@xs@newmacro@0}%
}

% #1 : dernier num\'ero de l'argument devant être d\'etokenis\'e
% #2 : nom de la macro publique
% #3 : argument optionnel (vide si pas d'arg optionnel)
% #4 : nombre d'arguments obligatoires
% #5 : utilisation de testopt (1 si oui, 0 si non)
% #6 : code de la macro
\def\@xs@newmacro@#1#2#3#4#5{%
	\edef\@xs@reserved@A{@xs@\expandafter\@gobble\string#2}%
	\edef\@xs@reserved@C{\expandafter\noexpand\csname\@xs@reserved@A @\ifx\@empty#3\@empty @\fi\endcsname}%
	\edef\@xs@reserved@B{%
		\ifx\@empty\@xs@reserved@D
			\def\noexpand#2{\noexpand\@ifstar
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@detokenize\expandafter\noexpand\@xs@reserved@C}%
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
			}%
		\else
			\def\noexpand#2{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
		\fi
		\ifx\@empty#3\@empty
		\else
			\def\expandafter\noexpand\@xs@reserved@C{%
				\noexpand\@testopt{\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname}{\ifx\@xs@def\@xs@ledef#3\else\unexpanded{#3}\fi}}%
		\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit :
	% si #3 est vide : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@@}}
	% si #3 existe   : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@}}
	%                  \@xs@NOM@{\@testopt{\@xs@NOM@@}{#3}}}
	\long\@xs@reserved@B
	\ifx\@empty#3\@empty
		\@xs@BuildLines1{#4}{#3}{#1}%
		\@xs@DefArg{#4}%
	\else
		\expandafter\@xs@BuildLines\expandafter1\expandafter{\number\numexpr#4+1}{#3}{#1}%
		\@xs@DefArg@{#4}%
	\fi
	\edef\@xs@reserved@B{\def\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname\@xs@myarg}%
	\edef\@xs@reserved@C{\unexpanded\expandafter{\@xs@newlines}\edef\noexpand\@xs@call}%
	\edef\@xs@reserved@D{%
		\noexpand\noexpand\expandafter\noexpand\csname\@xs@reserved@A\endcsname\unexpanded\expandafter{\@xs@newargs}%
	}%
	\ifnum#5=\@ne\edef\@xs@reserved@D{\noexpand\noexpand\noexpand\@testopt{\unexpanded\expandafter{\@xs@reserved@D}}{}}\fi
	\@xs@edefaddtomacro\@xs@reserved@C{{\unexpanded\expandafter{\@xs@reserved@D}}\noexpand\@xs@call}%
	\@xs@edefaddtomacro\@xs@reserved@B{{\unexpanded\expandafter{\@xs@reserved@C}}}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def\@xs@NOM@@[##2]##3##4##5{%
	%          \@xs@def\@xs@arg@i{##2}\@xs@assign\@xs@arg@ii{##3}\@xs@assign\@xs@arg@iii{##4}\@xs@asign\@xs@arg@iv{##5}%
	% si #5=0: \edef\@xs@call{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}%
	% si #5=1: \edef\@xs@call{\noexpand\@testopt{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@i}{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}{}}%
	%          \@xs@call}
	\long\@xs@reserved@B
	\edef\@xs@reserved@B{%
		\def\expandafter\noexpand\csname\@xs@reserved@A\endcsname
			\@xs@myarg\ifnum#5=\@ne[\unexpanded{##}\number\numexpr\ifx\@empty#3\@empty#4+1\else#4+2\fi]\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def \@xs@NOM[##2]##3##4##5[##6]{#6}
	\long\@xs@reserved@B
}

% macro g\'en\'erique qui lit \@xs@reserved@C us par us
% 3 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atbegingroup      (un groupe vient d'être ouvert)
% \@xs@atnextsyntaxunit  (la future US n'est pas un groupe)
\def\@xs@read@reserved@C{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@read@reserved@C
		\@xs@exploregroups
		\ifx\bgroup\@xs@toks
			\advance\integerpart\@ne
			\begingroup
				\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
				\@xs@manage@groupID
				\let\@xs@nestlevel\@ne
				\integerpart\z@
				\@xs@atbegingroup
		\else
			\global\advance\decimalpart\@ne
			\@xs@atnextsyntaxunit
		\fi
		}%
	\@xs@next
}

% macro g\'en\'erique qui lit \@xs@reserved@D en proc\'edant \`a des tests avec \IfBeginWith
% 2 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atoccurfound      (une occurrence a \'et\'e trouv\'ee)
\def\@xs@read@reserved@D{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}%
		{\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
			{\expandafter\@xs@reserved@D\expandafter}\expandafter{\@xs@reserved@E}%
			{\global\advance\decimalpart\@ne
			\let\@xs@reserved@D\@xs@reserved@A
			\@xs@atoccurfound
			}%
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@A
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
			\let\@xs@next\@xs@read@reserved@D
			\@xs@exploregroups
			\ifx\bgroup\@xs@toks
				\advance\integerpart\@ne
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@D\@xs@reserved@A
					\@xs@manage@groupID
					\let\@xs@reserved@C\@empty
					\let\@xs@nestlevel\@ne
					\integerpart\z@
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro\StrRemoveBraces{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\let\@xs@reserved@B\@empty
	\let\@xs@nestlevel\z@
	\@xs@StrRemoveBraces@i
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#2}%
}

\def\@xs@StrRemoveBraces@i{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@B}%
			\let\@xs@next\@xs@StrRemoveBraces@i
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@StrRemoveBraces@i
		\ifx\bgroup\@xs@toks
			\ifx\@xs@exploregroups\relax% on explore les groupes ?
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
					\let\@xs@nestlevel\@ne
					\integerpart\z@
					\let\@xs@reserved@B\@empty
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\@xs@reserved@A
			\fi
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
		\fi
		}%
	\@xs@next
}

% \@xs@cutafteroccur coupe l'argument #1 apr\`es la #3\`eme occurrence de #2
% \@xs@reserved@C : contient ce qui se trouve avant cette occurrence
% \@xs@reserved@D : contient ce qui se trouve avant cette occurrence y compris cette occurrence
% \@xs@reserved@E : contient ce qui se trouve apr\`es l'occurrence
% si l'occurrence n'existe pas ou qu'un des arguments est vide, toutes les chaines renvoy\'ees sont vides
\long\def\@xs@cutafteroccur#1#2#3{%
	\ifnum#3<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
		{\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
		}
		{\@xs@cutafteroccur@i{#1}{#2}{#3}}%
}
	
\long\def\@xs@cutafteroccur@i#1#2#3{%
	\def\@xs@reserved@D{#1}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#2}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\ifnum\decimalpart=\numexpr(#3)\relax % occurrence trouv\'ee ?
		\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\@xs@argument@A}%
	\else
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
	\fi
}

\@xs@newmacro*3\IfSubStr{1}{2}{0}{%
	\def\@xs@argument@A{#2}\def\@xs@argument@B{#3}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur
	\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter{\@xs@argument@B}{#1}%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*2\IfBeginWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@secondoftwo
		}
		{\def\@xs@next{%
			\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
				{\expandafter\@xs@argument@A\expandafter}\expandafter
				{\@xs@argument@B}}%
		}%
	\@xs@next
}

\long\def\@xs@IfBeginWith@i#1#2{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@firstoftwo% #2 est vide, tous les tests sont pass\'es avec succ\`es : on renvoie #3
		}
		{\expandafter\@xs@ifempty\expandafter{\@xs@argument@A}%
			{\let\@xs@next\@secondoftwo% #1 est vide, c'est que #2 est + long que #1 : on renvoie #4
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
			\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
			\ifx\@xs@reserved@A\@xs@reserved@B% il y a \'egalit\'e...
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A% on enl\`eve les 1ere unit\'es syntaxiques
				\def\@xs@next{% et on recommence avec ces arguments racourcis d'1 unit\'e syntaxique
					\expandafter\expandafter\expandafter\@xs@IfBeginWith@i
					\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}}%
			\else
				\let\@xs@next\@secondoftwo
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro*2\IfEndWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\@xs@ifempty{#2}%
		{\let\@xs@reserved@A\@secondoftwo
		}
		{\expandafter\expandafter\expandafter\@xs@StrCount
			\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter
			{\@xs@argument@B}[\@xs@reserved@A]%
		\ifnum\@xs@reserved@A=\z@
			\let\@xs@reserved@A\@secondoftwo
		\else
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
				{\let\@xs@reserved@A\@firstoftwo}
				{\let\@xs@reserved@A\@secondoftwo}%
		\fi
		}%
	\@xs@reserved@A
}

\@xs@newmacro*4\IfSubStrBefore{1,1}{3}{0}{\@xs@IfSubStrBefore@i[#1]{#2}{#3}{#4}}

\def\@xs@IfSubStrBefore@i[#1,#2]#3#4#5{%
	\def\@xs@reserved@C{#3}%
	\ifx\@xs@exploregroups\relax% si on explore les groupes
		\let\@xs@reserved@B\@empty
		\let\@xs@nestlevel\z@
		\@xs@StrRemoveBraces@i% on retire les accolades
		\let\@xs@reserved@C\@xs@reserved@B
	\fi
	\def\@xs@reserved@A{#5}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#2}%
	\def\@xs@reserved@A{#4}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#1}%
	\global\let\groupID\@empty
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*4\IfSubStrBehind{1,1}{3}{0}{\@xs@IfSubStrBehind@i[#1]{#2}{#3}{#4}}

\long\def\@xs@IfSubStrBehind@i[#1,#2]#3#4#5{\@xs@IfSubStrBefore@i[#2,#1]{#3}{#5}{#4}}

\long\def\@xs@formatnumber#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#1}%
		{\def#2{0X}% si vide, renvoie 0X
		}
		{\@xs@returnfirstsyntaxunit{#1}\@xs@reserved@A
		\def\@xs@reserved@B{+}%
		\ifx\@xs@reserved@A\@xs@reserved@B
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@C
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			 	{\def#2{+0X}}
			 	{\expandafter\def\expandafter#2\expandafter{\expandafter+\expandafter0\@xs@reserved@C}}%
		\else
			\def\@xs@reserved@B{-}%
			\ifx\@xs@reserved@A\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
				\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
					{\def#2{-0X}}%
					{\expandafter\def\expandafter#2\expandafter{\expandafter-\expandafter0\@xs@reserved@A}}%
			\else
				\expandafter\def\expandafter#2\expandafter{\expandafter0\@xs@argument@A}%
			\fi
		\fi
		}%
}

\@xs@newmacro\IfInteger{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\let\@xs@after@intpart\@xs@afterinteger
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\ifnum\decimalpart=\z@
			\let\@xs@next\@firstoftwo% partie décimale constituée de 0 --> seul cas où on renvoie vrai
		\else
			\let\@xs@afterinteger\@xs@after@intpart
			\let\@xs@next\@secondoftwo
		\fi
	\else
		\let\@xs@afterinteger\@xs@after@intpart
		\let\@xs@next\@secondoftwo
	\fi
	\@xs@next
}

\@xs@newmacro\IfDecimal{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}

\long\def\@xs@defafterinteger#1\relax\@xs@nil{\def\@xs@afterinteger{#1}}

\def\@xs@testdot{%
	\let\xs@decsep\@empty
	\@ifnextchar.%
		{\def\xs@decsep{.}\@xs@readdecimalpart}%
		{\@xs@testcomma}%
}

\def\@xs@testcomma{%
	\@ifnextchar,%
		{\def\xs@dessep{,}\@xs@readdecimalpart}%
		{\@xs@endnumber}%
}

\long\def\@xs@readdecimalpart#1#2\@xs@nil{%
	\ifx\@empty#2\@empty
		\def\@xs@reserved@A{0X}%
	\else
		\def\@xs@reserved@A{0#2}%
	\fi
	\afterassignment\@xs@defafterinteger\decimalpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@endnumber\@xs@afterinteger\@xs@nil
}

\long\def\@xs@endnumber#1\@xs@nil{\def\@xs@afterdecimal{#1}}

% test d'\'egalit\'e sur des chaines (et des chaines contenant des nombres)
\long\def\@xs@IfStrEqFalse@i#1#2{\let\@xs@reserved@A\@secondoftwo}
\long\def\@xs@IfStrEqFalse@ii#1#2{% renvoie vrai si les 2 arg sont d\'ecimaux et s'ils sont \'egaux, faux sinon
	\@xs@IfDecimal{#1}%
		{\@xs@IfDecimal{#2}%
			{\ifdim#1pt=#2pt
				\let\@xs@reserved@A\@firstoftwo
			\else
				\let\@xs@reserved@A\@secondoftwo
			\fi% les 2 sont d\'ecimaux : on fait le test
			}%
			{\let\@xs@reserved@A\@secondoftwo}% un seul est d\'ecimal
		}%
		{\let\@xs@reserved@A\@secondoftwo}% #1 n'est pas d\'ecimal
}

\long\def\@xs@TestEqual#1#2{% teste si les 2 arguments sont \'egaux
	\def\@xs@reserved@A{#1}\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\let\@xs@reserved@A\@firstoftwo% \'egalit\'e parfaite des 2 chaines
	\else
		\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}%
	\fi
	\@xs@reserved@A
}

\@xs@newmacro*2\IfStrEq{}{2}{0}{% teste si les deux chaines sont \'egales
	\let\@xs@reserved@D\@xs@IfStrEqFalse@i
	\@xs@TestEqual{#1}{#2}%
}

\@xs@newmacro*2\IfEq{}{2}{0}{% teste si les 2 arguments (chaine ou nombre) sont \'egaux
	\let\@xs@reserved@D\@xs@IfStrEqFalse@ii
	\@xs@TestEqual{#1}{#2}%
}

\def\IfStrEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfStrEq*}\@xs@IfStrCase}%
		{\def\@xs@reserved@E{\IfStrEq}\@xs@IfStrCase}%
}

\long\def\@xs@IfStrCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\def\IfEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfEq*}\@xs@IfEqCase}%
		{\def\@xs@reserved@E{\IfEq}\@xs@IfEqCase}%
}

\long\def\@xs@IfEqCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\long\def\@xs@IfStringCase#1#2[#3]{%
	\long\def\@xs@testcase##1##2##3\@xs@nil{% lit les 2 premieres unit\'es syntaxiques dans ##1 et ##2. Les autres dans ##3
		\@xs@reserved@E{#1}{##1}%
			{##2}% le test est positif, on ex\'ecute le code correspondant
			{\@xs@ifempty{##3}%
			 	{#3}% s'il n'y a plus de cas, on ex\'ecute le code <autres cas>
				{\@xs@testcase##3\@xs@nil}% sinon, on recommence avec ce qui reste
			 }%
	}%
	\@xs@testcase#2\@xs@nil
}

% Renvoie ce qui est \`a gauche de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBefore{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
}

% Renvoie ce qui est \`a droite de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBehind{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#4}%
}

% Renvoie ce qui est strictement compris entre les occurrences n°#1 et n°#2
% des chaines #4 et #5 dans la chaine #3
\@xs@newmacro*4\StrBetween{1,1}{3}{1}{\@xs@StrBetween@i[#1]{#2}{#3}{#4}[#5]}

\long\def\@xs@StrBetween@i[#1,#2]#3#4#5[#6]{%
	\begingroup
		\noexploregroups
		\@xs@cutafteroccur{#3}{#5}{#2}%
		\expandafter\@xs@cutafteroccur\expandafter{\@xs@reserved@C}{#4}{#1}%
		\expandafter
	\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#6}%
	\global\let\groupID\@empty
}

\def\exploregroups{\let\@xs@exploregroups\relax}

\def\noexploregroups{\def\@xs@exploregroups{\let\@xs@toks0\relax}}

\def\saveexploremode{\let\@xs@saveexploremode\@xs@exploregroups}

\def\restoreexploremode{\let\@xs@exploregroups\@xs@saveexploremode}

% Remplace les #1 premi\`eres occurences de la chaine #3
% par la chaine #4 dans la chaine #2
\@xs@newmacro\StrSubstitute{0}{3}{1}{%
	\def\@xs@reserved@D{#2}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#3}%
	\def\@xs@argument@C{#3}\def\@xs@argument@D{#4}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum#1<\@ne
			\let\@xs@reserved@A\@xs@argument@D
		\else
			\ifnum\decimalpart>#1
				\let\@xs@reserved@A\@xs@argument@C
			\else
				\let\@xs@reserved@A\@xs@argument@D
			\fi
		\fi
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
		\@xs@read@reserved@D
	}%
	\@xs@ifempty{#3}%
		{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#5}%
		}
		{\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#5}%
		}%
}

% Supprime les #1 premi\`eres occurrences de #3 dans #2
\@xs@newmacro\StrDel{0}{2}{1}{\@xs@StrSubstitute[#1]{#2}{#3}{}[#4]}

\def\@xs@exitallgroups{\ifnum\@xs@nestlevel>\z@\endgroup\expandafter\@xs@exitallgroups\fi}

% Compte combien d'unit\'es syntaxiques contient la chaine #1 ?
\@xs@newmacro\StrLen{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\decimalpart\z@
	\let\@xs@nestlevel\z@
	\gdef\groupID{0}%
	\let\@xs@atbegingroup\relax
	\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
	\let\@xs@atnextsyntaxunit\relax
	\@xs@read@reserved@C
	\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#2}%
}

% Macro interne fermant autant de groupes que n\'ecessaire pour trouver une unit\'e syntaxique derri\`ere
\def\@xs@continuetonext{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel>\z@
			\expandafter\endgroup\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}% on concat\`ene
			\expandafter\expandafter\expandafter\@xs@continuetonext% on recommence
		\fi}
		\relax
}%

\def\@xs@manage@groupID{%
	\begingroup\def\@xs@reserved@A{0}%
	\ifx\@xs@reserved@A\groupID% si on arrive du groupe de niveau 0
		\endgroup
		\xdef\groupID{\number\integerpart}% on met simplement le niveau
	\else
		\endgroup
		\expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter\groupID\expandafter\expandafter\expandafter{\expandafter\groupID\expandafter,\number\integerpart}%
	\fi
}

% Cette macro coupe la chaine #1 apr\`es l'unit\'e syntaxique n°#2
\def\StrSplit{%
	\@ifstar
		{\let\@xs@reserved@E\@xs@continuetonext\StrSpl@t}%
		{\let\@xs@reserved@E\relax\StrSpl@t}%
}

\@xs@newmacro\StrSpl@t{}{2}{0}{\@xs@StrSplit@i{#2}{#1}\@xs@StrSplit@ii}

% Cette macro interne coupe la chaine #2 apr\`es l'unit\'e syntaxique n°#1
% Le d\'ebut est assign\'e dans \@xs@reserved@B et la fin dans \@xs@reserved@C
\long\def\@xs@StrSplit@i#1#2{%
	\def\@xs@reserved@D{#1}%
	\def\@xs@reserved@C{#2}%
	\let\@xs@reserved@B\@empty
	\global\let\groupID\@empty
	\ifnum#1>\z@
		\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
			\@xs@read@reserved@C
		}%
		\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
		\def\@xs@atnextsyntaxunit{%
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
			\ifnum\decimalpart=\@xs@reserved@D\relax
				\ifx\@xs@reserved@C\@empty\@xs@reserved@E\fi
				\global\let\@xs@reserved@B\@xs@reserved@B
				\global\let\@xs@reserved@C\@xs@reserved@C
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
}

\def\@xs@StrSplit@ii#1#2{\let#1\@xs@reserved@B\let#2\@xs@reserved@C}

% StrCut[n]{<texte>}{<motif>}\macroA\macroB
% \macroA reçoit ce qui se trouve avant la n ème occurrence <motif> dans <texte>
% \macroB reçoit ce qui est après cette n ème occurrence
\@xs@newmacro*3\StrCut{1}{2}{0}{%
	\@xs@ifempty{#3}%
		{\global\let\groupID\@empty
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		}
		{\ifnum#1<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
			{\@xs@StrCut@ii{#2}{#3}1}
			{\@xs@StrCut@ii{#2}{#3}{#1}}%
		}%
	\@xs@StrCut@iii
}

\long\def\@xs@StrCut@ii#1#2#3{%
	\def\@xs@reserved@D{#1}%
	\let\@xs@reserved@C\@empty
	\def\@xs@reserved@E{#2}%
	\decimalpart\z@\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi
	}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter
	\def
		\expandafter\expandafter\expandafter
	\@xs@reserved@D
		\expandafter\expandafter\expandafter
	{\expandafter\@xs@reserved@C\@xs@argument@A}%
}

\long\def\@xs@StrCut@iii#1#2{\let#1\@xs@reserved@C\let#2\@xs@reserved@E}

% De la chaine #1, renvoie ce qui se trouve entre les positions
%  #2 et #3, unit\'es syntaxiques aux positions compris !
\@xs@newmacro\StrMid{}{3}{1}{%
	\begingroup
		\noexploregroups
		\let\@xs@reserved@E\relax
		\@xs@StrSplit@i{#3}{#1}%
		\edef\@xs@reserved@C{\number\numexpr#2-1}%
		\let\@xs@reserved@E\relax
		\expandafter\expandafter\expandafter\@xs@StrSplit@i\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@B}%
	\expandafter\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
	\global\let\groupID\@empty
}

% supprime #2 unit\'es syntaxiques \`a gauche dans la chaine #1
\@xs@newmacro\StrGobbleLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

% extrait de #1 la chaine \`a gauche de longueur #2
\@xs@newmacro\StrLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% supprime #2 unit\'es syntaxiques \`a droite dans la chaine #1
\@xs@newmacro\StrGobbleRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% renvoie #2 unit\'es syntaxiques \`a la droite de la chaine #1
\@xs@newmacro\StrRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

\@xs@newmacro\StrChar{}{2}{1}{%
	\let\@xs@reserved@B\@empty
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\ifnum#2>\z@
		\def\groupID{0}\let\@xs@nestlevel\z@\integerpart\z@\decimalpart\z@
		\let\@xs@atbegingroup\relax
		\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
		\def\@xs@atnextsyntaxunit{%
			\ifnum\decimalpart=\@xs@reserved@D% la n i\`eme US est atteinte ?
				\global\let\@xs@reserved@B\@xs@reserved@A% on capture l'US en cours qui est celle cherch\'ee
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@B}%
		{\global\let\groupID\@empty}
		\relax
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% Combien de fois compte t-on #2 dans #1 ?
\@xs@newmacro\StrCount{}{2}{1}{%
	\def\@xs@reserved@D{#1}\def\@xs@reserved@E{#2}\let\@xs@reserved@C\@empty
	\@xs@ifempty{#2}%
		{\@xs@ReturnResult{0}{#3}}
		{\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
			\@xs@read@reserved@D
		}%
		\def\@xs@atoccurfound{\let\@xs@reserved@C\@empty\@xs@read@reserved@D}%
		\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#3}%
		}%
}

% renvoie la position de l'occurrence #1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro\StrPosition{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\let\@xs@reserved@E\groupID
	\ifx\@xs@reserved@C\@xs@reserved@D
		\@xs@ReturnResult{0}{#4}%
		\let\@xs@reserved@E\@empty
	\else
		\expandafter\@xs@StrLen\expandafter{\@xs@reserved@C}[\@xs@reserved@C]%
		\expandafter\@xs@ReturnResult\expandafter{\number\numexpr\@xs@reserved@C+1}{#4}%
	\fi
	\global\let\groupID\@xs@reserved@E
}

\def\comparestrict{\let\@xs@comparecoeff\@ne}

\def\comparenormal{\let\@xs@comparecoeff\z@}

\def\savecomparemode{\let\@xs@saved@comparecoeff\@xs@comparecoeff}

\def\restorecomparemode{\let\@xs@comparecoeff\@xs@saved@comparecoeff}

% Compare les deux arguments #1 et #2
% Renvoie 0 s'ils sont \'egaux et renvoie la
% position de la premiere unit\'e syntaxiques diff\'erente sinon
\@xs@newmacro*2\StrCompare{}{2}{1}{%
	\def\@xs@reserved@A{#1}%
	\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@B\@xs@reserved@A
		\@xs@ReturnResult{0}{#3}%
	\else
		\def\@xs@next{\@xs@StrCompare@i{#1}{#2}{#3}}%
		\expandafter\@xs@next
	\fi
}

\long\def\@xs@StrCompare@i#1#2#3{%
	\def\@xs@StrCompare@iii##1{%
		\let\@xs@reserved@A\@empty
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@reserved@A{*\@xs@comparecoeff}}%
			{\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
				{\def\@xs@reserved@A{*\@xs@comparecoeff}}
				\relax
			}%
		\def\@xs@next{%
			\expandafter\@xs@ReturnResult\expandafter
			{\number\numexpr##1\@xs@reserved@A\relax}{#3}%
		}%
	}%
	\def\@xs@StrCompare@ii##1{% ##1 est la position
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@B
		\ifx\@xs@reserved@B\@xs@reserved@A
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
				{\@xs@StrCompare@iii{##1}% les 2 unit\'es syntaxiques sont \'egales, on renvoie la position
				}
				{\def\@xs@next{\expandafter\@xs@StrCompare@ii\expandafter{\number\numexpr##1+1}}% les 2 unit\'es syntaxiques sont \'egales et non vides, on recommence
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
				}%
		\else% les 2 unit\'es syntaxiques sont diff\'erentes : on renvoie la position
			\@xs@StrCompare@iii{##1}%
		\fi
		\@xs@next
	}%
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\@xs@StrCompare@ii1%
}

\@xs@newmacro\StrFindGroup{}{2}{1}{%
	\def\@xs@reserved@A{#2}\def\@xs@reserved@B{0}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\def\@xs@next{\@xs@ReturnResult{{#1}}{#3}}%
	\else
		\def\@xs@next{\@xs@StrFindGroup@i{#1}{#2}[#3]}%
	\fi
	\@xs@next
}

\long\def\@xs@StrFindGroup@i#1#2[#3]{%
	\def\@xs@StrFindGroup@ii{%
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@next{\@xs@ReturnResult{}{#3}}% s'il ne reste plus rien, on renvoie vide
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@D
			\ifx\bgroup\@xs@toks% si la 1\`ere unit\'e syntaxique est un groupe explicite
				\advance\decimalpart\@ne% on augmente le compteur
				\ifnum\decimalpart=\@xs@reserved@A% on est au groupe cherch\'e lors de la profondeur courante ?
					\ifx\@empty\@xs@reserved@B% on est \`a la profondeur maximale ?
						\def\@xs@next{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#3}}% on renvoie ce groupe
					\else% sinon
						\expandafter\def\expandafter\@xs@next\expandafter{\expandafter\@xs@StrFindGroup@i\@xs@reserved@D}% on recommence avec ce groupe
						\expandafter\@xs@addtomacro\expandafter\@xs@next\expandafter{\expandafter{\@xs@reserved@B}[#3]}% et les profondeurs de recherche restantes
					\fi
				\else
					\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
					\let\@xs@next\@xs@StrFindGroup@ii
				\fi
			\else
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\let\@xs@next\@xs@StrFindGroup@ii
			\fi
			}%
		\@xs@next
	}%
	\@xs@extractgroupnumber{#2}\@xs@reserved@A\@xs@reserved@B
	\decimalpart\z@
	\ifnum\@xs@reserved@A>\z@\def\@xs@reserved@C{#1}\else\let\@xs@reserved@C\@empty\fi
	\@xs@StrFindGroup@ii
}

\def\@xs@extractgroupnumber#1#2#3{%
	\def\@xs@extractgroupnumber@i##1,##2\@xs@nil{\def#2{##1}\def#3{##2}}%
	\@xs@extractgroupnumber@i#1,\@xs@nil
	\ifx\@empty#3\else\@xs@extractgroupnumber@i#1\@xs@nil\fi
}

\def\expandingroups{\let\@xs@expandingroups\exploregroups}

\def\noexpandingroups{\let\@xs@expandingroups\noexploregroups}

\def\StrExpand{\@testopt{\@xs@StrExpand}{1}}
\long\def\@xs@StrExpand[#1]#2#3{%
	\begingroup
		\@xs@expandingroups
		\ifnum#1>\z@
			\integerpart#1\relax
			\decimalpart\z@
			\gdef\groupID{0}%
			\let\@xs@nestlevel\z@
			\def\@xs@atendofgroup{%
				\expandafter\endgroup
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
				\@xs@read@reserved@C
			}%
			\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
			\def\@xs@atnextsyntaxunit{%
				\expandafter\expandafter\expandafter\@xs@addtomacro
				\expandafter\expandafter\expandafter\@xs@reserved@B
				\expandafter\expandafter\expandafter{\@xs@reserved@A}%
			}%
			\def\@xs@reserved@C{#2}%
			\@xs@StrExpand@i{#1}% Appel de la macro r\'ecursive
		\else
			\def\@xs@reserved@B{#2}%
		\fi
		\global\let\@xs@reserved@B\@xs@reserved@B
	\endgroup
	\let#3\@xs@reserved@B
	\global\let\groupID\@empty
}

\long\def\@xs@StrExpand@i#1{%
	\ifnum#1>\z@
		\let\@xs@reserved@B\@empty
		\@xs@read@reserved@C
		\let\@xs@reserved@C\@xs@reserved@B
		\def\@xs@reserved@A{\expandafter\@xs@StrExpand@i\expandafter{\number\numexpr#1-1}}%
	\else
		\let\@xs@reserved@A\relax
	\fi
	\@xs@reserved@A
}

\def\scancs{\@testopt{\@xs@scancs}{1}}
\long\def\@xs@scancs[#1]#2#3{%
	\@xs@StrExpand[#1]{#3}{#2}%
	\edef#2{\detokenize\expandafter{#2}}%
}

% Restaure le code de @
\catcode`\@=\CurrentAtCatcode\relax

% D\'efinit le d\'elimiteur verb
% d\'efinit les diff\'erents modes et les m\'emorise
\setverbdelim{|}%
\fullexpandarg\saveexpandmode
\comparenormal\savecomparemode
\noexploregroups\saveexploremode
\expandingroups

\endinput
%
% Historique
%------------------------------------------------------------------------------
%% v1.0    4/7/2008 : - Package achev\'e.
%          7/7/2008 : - Package publi\'e sur CTAN.
%------------------------------------------------------------------------------
% v1.1    15/8/2008
%   - Le package ne n\'ecessite plus LaTeX et est d\'esormais utilisable sous
%     Plain eTeX.
%   - Ajout des macros \IfInteger et \IfDecimal.
%     Pour cette derni\`ere, la partie enti\`ere et la partie d\'ecimale sont
%     r\'ecup\'erables dans les compteurs \integerpart et \decimalpart. Ce
%     qu'il reste apr\`es qu'un caract\`ere non attendu soit rencontr\'e est
%     dispo dans \@xs@remainafterdecimal
%   - Correction d'un bug dans \tokenize :
%        suppression de l'expansion avec \normalexpandarg pour \'eviter le bug
%        avec les lettres accentu\'ees dans l'exemple : \tokenize\aa{\'e\`u}
%   - Am\'elioration du code de la plupart des macros.
%   - \'Ecriture d'une routine \@xs@newmacro d\'efinissant les  macros.
%   - Suppression de tous les compteurs grace \`a \numexpr.
%   - Nouvelles fonctionnalit\'es internes dans :
%      \IfSubStr
%        ajout des chaines se trouvant avant et apr\`es l'occurrence test\'ee
%        dans les sc \@xs@behind@IfSubStr et \@xs@before@IfSubStr
%      \StrCount
%        a) ajout de ce qui se trouve apr\`es la derni\`ere occurrence dans la
%           sc \@xs@StrCount@afterlastocccur
%        b) la macro ne d\'epend plus d'aucune autre
%------------------------------------------------------------------------------
% v1.2    23/8/2008
%   - Am\'elioration du code de \StrMid \StrGobbleLeft, \StrLeft,
%     \StrGobbleRight et \StrRight \`a l'aide de la nouvelle macro
%     \@xs@StrSplit@i
%   - Nouveau test \IfStrEq qui compare 2 chaines
%   - Nouveau test \IfEq qui compare 2 chaines (ou 2 nombres si les 2 chaines
%     contiennent un nombre)
%   - Correction d'un bug dans \@xs@formatnumber. La macro n'envisageait pas le
%     cas o\`u son argument \'etait vide ce qui faiasait planter
%     \IfDecimal{}{V}{F} et \IfInteger{}{V}{F}
%------------------------------------------------------------------------------
% v1.3    21/9/2008
%  - Am\'elioration du code, mise en place de r\'ecursivit\'es terminales dans
%    toutes les macros r\'ecursives, simplification de \@xs@TestEqual en
%    utilisant \ifx
%  - Nouvelles macros \IfStrEqCase et \IfEqCase
%      Teste si une chaîne est \'egale \`a plusieurs cha\^ines donn\'ee et
%      ex\'ecute un code sp\'ecifique
%  - Cr\'eation de la macro publique \StrSplit
%      Coupe la chaine en 2 \`a une position donn\'ee
%  - Nouvelle macro \StrCompare
%      Compare 2 chaînes et renvoie la position du 1er caract\`ere diff\'erent.
%      Renvoie 0 si elles sont \'egales.
%------------------------------------------------------------------------------
% v1.3a   29/9/2008
%  - Correction d'un bug : \expandafter#1
%    dans les macros \IfSubStrBefore et \StrBetween qui buggue si #1 est un
%    nombre > 9 !
%  - R\'e \'ecriture de \@xs@returnfirstsyntaxunit et \@gobble qui
%    deviennent purement d\'eveloppables.
%  - R\'e \'ecriture de \StrLen
%  - Nouvelle macro interne \@xs@cutafteroccur
%      Coupe la chaine apr\`es la ni\`eme occurrence d'une sous chaine.
%  - Code am\'elior\'e de \StrMid, \StrLeft, \StrGobbleLeft, \StrRight,
%    \StrGobbleRight grace \`a \@xs@cutafteroccur
%------------------------------------------------------------------------------
% v1.4   4/11/2008
%  - xstring traite ses arguments par unit\'e syntaxique, et donc toutes les
%    macros internes ont \'et\'e r\'e-\'ecrites \`a cette fin.
%  - Le manuel a \'et\'e r\'e-\'ecrit, rendu plus clair et mieux structur\'e.
%  - Nouvelle fonctionnalit\'e : \expandarg
%      le 1er lex\`eme de chaque argument est 1-d\'evelopp\'e avant que la
%      macro ne soit appel\'ee. Si un argument comporte plus qu'1 lex\`eme,
%      il faut passer par \scancs*[1] pour 1-d\'evelopper toutes les unit\'es
%      syntaxiques.
%  - Correction de 2 erreurs dans le manuel anglais :  0 est la valeur par
%    d\'efaut dans \StrSubstitute et \StrDel
%  - Coh\'erence dans les nom des s\'equences de contr\^oles temporaires qui
%    sont d\'esormais : \@xs@reserved@A \`a \@xs@reserved@E
%------------------------------------------------------------------------------
% v1.4a  12/11/2008
%  - Correction d'un bug dans \@xs@StrSplit dans le cas o\`u l'argument
%     num\'erique est <1 : la 1ere coupure doit être vide et le seconde doit
%     être \'egale \`a l'argument.
%------------------------------------------------------------------------------
% v1.4b  16/11/2008
%  - Correction de 2 bugs dans \@xs@returnfirstsyntaxunit
%------------------------------------------------------------------------------
% v1.5   31/12/2008
%  - Nouvelles fonctionnalit\'es dans la recherche de groupes par un
%    identificateur caract\'erisant leur imbrication. Impl\'ementation de :
%      1) \StrFindGroup
%      2) \groupID
%  - Ajout des nouvelles macros g\'en\'eriques \@xs@read@reserved@C et
%    \@xs@read@reserved@D
%  - Correction d'un bug dans \StrSplit : \StrSplit{{a}bc}{1}[\truc] faisait
%    que \truc contenait «a{a}».
%  - Correction d'un bug dans \@xs@newmacro : l'argument optionnel \'etait
%    d\'etok\'enis\'e \`a tort dans les macros \'etoil\'ees.
%  - Dans \@xs@newmacro, on doit choisir le num\'ero du dernier argument devant
%    être d\'etok\'enis\'e dans le cas d'une macro \'etoil\'ee (sachant que
%     l'argument optionnel ne l'est jamais)
%------------------------------------------------------------------------------
% v1.5a  09/2/2009
%  - Nouvelle macro \StrExpand, sensible au mode d'exploration. La macro est
%    indépendante du mode d'exploration et dispose de ses propres commandes
%    d'exploration : \expandingroups et \noexpandingroups
%  - R\'e-\'ecriture de \scancs, qui devient triviale puisque d\'ependant de
%    \StrExpand. Il n'y a plus de version \'étoil\'ee et d\'esormais, \scancs
%    est sensible au mode d'exploration.
%  - Correction d'un bug dans \IfInteger : \IfInteger{2.0}{V}{F} affichait F
%  - Correction de bugs : mettre \let\@xs@reserved@E\relax avant d'appeler
%    \@xs@StrSplit@i
%  - Suppression des messages d'erreur, de warning et d'info. xstring devient
%    donc silencieux ;)
%  - Passage de 3 \'a 2 compteurs
%  - Le manuel est d\'esormais plus color\'e, en esp\'erant qu'il sera un peu
%    plus agr\'eable \`a lire !
%------------------------------------------------------------------------------
% v1.5b  13/3/2009
%  - Modification d'un grand nombre de macros de telle sorte que vraiment
%    n'importe quel code peut d\'esormais \^etre plac\'e dans les arguments des
%    macros (comme par exemple des \if, \ifx ou autre, m\^eme sans leur \fi, ce
%    qui n'\'etait pas possible jusqu'alors)
%------------------------------------------------------------------------------
% v1.5c  05/6/2009
%  - Correction d'un bug dans \IfBeginWith : il faut appeler
%    \@xs@returnfirstsyntaxunit pour l'argument #2 puis pour l'argument #1 et
%    non pas l'inverse pour que \@xs@toks reflète ce qui se trouve dans #1
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit au cas où #1 commence
%    par un espace : mettre \@xs@toks à 0
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit :
%    \@xs@returnfirstsyntaxunit{{}}\truc
%    faisait que \truc se développait en un espace.
%  - Correction d'un bug dans \@xs@removefirstsyntaxunit où le cas
%    \@xs@removefirstsyntaxunit{ {b}}\truc
%    donnait \truc se développant en «b» au lieu de «{b}».
%------------------------------------------------------------------------------
% v1.5d  28/3/2010
%  - Correction d'un bug dans \IfInteger : \@xs@afterinteger ne donnait pas le
%    bon r\'esultat. Par exemple avec 1.23 il renvoyait {} au lieu de {.23}
%  - \xs@formatnumber ne detokenize plus ses arguments (que m'est-il pass\'e
%    par la t\^ete pour que je code un truc comme ca ?), et donc
%    \@xs@afterinteger et \@xs@afterdecimal ont des tokens ayant le bon
%    catcode
%------------------------------------------------------------------------------
% v1.6  24/10/2012
%  - Correction d'un bug dans \@xs@cutafteroccur au cas o\`u #3<1
%  - \IfDecimal ne \detokenize plus l'argument.
%  - Nouvelle version de \tokenize qui enlevait les accolades si son argument
%    \'etait entre accolades
%  - Nouvelle macro \StrCut
%  - \@xs@cutafteroccur@i ne produit plus d'espace indésirable si #3 était
%    évalué par \numexpr
%------------------------------------------------------------------------------
% v1.7  13/1/2013
%  - Correction d'un manque de rigueur dans les assignations concernant
%    \groupID : elles sont toutes globales d\'esormais
%  - Les macros de xstring sont \long
%------------------------------------------------------------------------------
% v1.7a 28/2/2013
%  - Correction d'un espace parasite dans \@xs@removefirstsyntaxunit
%------------------------------------------------------------------------------
% v1.7b 29/7/2013
%  - La date contenue dans \xstringdate est désormais conforme
%------------------------------------------------------------------------------
% v1.7c 13/10/2013 
%  - les macros impliquées dans \IfStrCase et \IfStrEqCase sont désormais \long
